Discovering Language-neutral Sub-networks in Multilingual Language Models

Multilingual pre-trained language models transfer remarkably well on cross-lingual downstream tasks. However, the extent to which they learn language-neutral representations (i.e., shared representations that encode similar phenomena across languages), and the effect of such representations on cross-lingual transfer performance, remain open questions. In this work, we conceptualize language neutrality of multilingual models as a function of the overlap between language-encoding sub-networks of these models. We employ the lottery ticket hypothesis to discover sub-networks that are individually optimized for various languages and tasks. Our evaluation across three distinct tasks and eleven typologically-diverse languages demonstrates that sub-networks for different languages are topologically similar (i.e., language-neutral), making them effective initializations for cross-lingual transfer with limited performance degradation.

==> LTH_Multilingual_LMs_EMNLP/1.abstract.tex <==


% Multilingual pre-trained language models %such as multilingual BERT~(mBERT) 
% perform remarkably well on cross-lingual transfer for downstream tasks.
% Despite the impressive performance of these systems, the extent to which they learn language-neutral representations (\ie, shared representations that encode similar phenomena across languages), and the effect of such representations on cross-lingual transfer performance, remain open questions.

% In this work, we conceptualize language neutrality of multilingual models as a function of the overlap between language-encoding sub-networks of these models. %Using mBERT as a foundation
% We employ the lottery ticket hypothesis to discover sub-networks that are individually optimized for various languages and tasks.
% Using three distinct tasks and eleven typologically-diverse languages in our evaluation, we show that the sub-networks found for different languages are quite similar. Additionally, they serve as effective initializations for other languages with limited performance degradation, supporting the idea that multilingual LMs jointly encode multiple languages in shared parameters.
% % We conclude that these models are comprised of language-neutral sub-networks shared among many languages, along with multiple ancillary language-specific sub-networks, with the former playing a more prominent role in cross-lingual performance.\footnote{We will make our code publicly available.}
% We conclude that these models are comprised of language-neutral sub-networks that are shared among many languages, %along with multiple ancillary language-specific sub-networks, 
% and that they play a prominent role in cross-lingual transfer performance.\footnote{We will make our code publicly available.}
% %Our code is public\footnote{\href{https://github.com/...}{https://github.com/...}}.


%%%%%% Take 2 %%%%%%%
% Multilingual pre-trained language models perform remarkably well on cross-lingual transfer for downstream tasks.
% Despite the impressive performance of these systems, the extent to which they learn language-neutral representations (\ie, shared representations that encode similar phenomena across languages), and the effect of such representations on cross-lingual transfer performance, remain open questions.

% In this work, we conceptualize language neutrality of multilingual models as a function of the overlap between language-encoding sub-networks of these models. %Using mBERT as a foundation
% We employ the lottery ticket hypothesis to discover sub-networks that are individually optimized for various languages and tasks.
% Using three distinct tasks and eleven typologically-diverse languages in our evaluation, we show that these discovered sub-networks are topologically similar, making them effective initializations for other languages with limited performance degradation. %, supporting the idea that multilingual LMs jointly encode multiple languages in shared parameters.
% % We conclude that these models are comprised of language-neutral sub-networks shared among many languages, along with multiple ancillary language-specific sub-networks, with the former playing a more prominent role in cross-lingual performance.\footnote{We will make our code publicly available.}
% We conclude that these models are comprised of language-neutral sub-networks that are shared among many languages, %along with multiple ancillary language-specific sub-networks, 
% and that they play a prominent role in these models' cross-lingual transfer performance.\footnote{We will make our code publicly available.}


Multilingual pre-trained language models transfer remarkably well on cross-lingual downstream tasks.
However, the extent to which they learn language-neutral representations (\ie, shared representations that encode similar phenomena across languages), and the effect of such representations on cross-lingual transfer performance, remain open questions.

In this work, we conceptualize language neutrality of multilingual models as a function of the overlap between language-encoding sub-networks of these models.
We employ the lottery ticket hypothesis to discover sub-networks that are individually optimized for various languages and tasks.
Our evaluation across three distinct tasks and eleven typologically-diverse languages demonstrates that sub-networks for different languages are topologically similar (\ie, language-neutral), making them effective initializations for cross-lingual transfer with limited performance degradation.\footnote{Our code is available at \href{https://github.com/negar-foroutan/multiLMs-lang-neutral-subnets}{https://github.com/negar-foroutan/multiLMs-lang-neutral-subnets}.}
% Code available at \href{https://github.com/negar-foroutan/multiLMs-lang-neutral-subnets}{https://github.com/negar-foroutan/multiLMs-lang-neutral-subnets}.
%, supporting the idea that multilingual LMs jointly encode multiple languages in shared parameters.
% We conclude that these models are comprised of language-neutral sub-networks shared among many languages, along with multiple ancillary language-specific sub-networks, with the former playing a more prominent role in cross-lingual performance.\footnote{We will make our code publicly available.}
% We conclude that these models are comprised of language-neutral sub-networks that are shared among many languages, %along with multiple ancillary language-specific sub-networks, 
% and that they play a prominent role in these models' cross-lingual transfer performance.


% Multilingual pre-trained language models such as multilingual BERT~(mBERT) perform remarkably well on cross-lingual transfer for downstream tasks.
% Despite it's impressive performance, our understanding of mBERT's language neutrality and its role in achieving such performance is still obscure.
% In this work we shed light on mBERT's language neutrality by employing the lottery ticket hypothesis to obtain pruned sub-networks for various languages and tasks.
% Using three distinct tasks and eleven typologically-diverse languages in our evaluation, we show that the sub-networks found for different languages are similar, supporting the idea that mBERT is an interlingua.
% We conclude that mBERT is comprised of two language-specific and language-neutral components, with the latter playing a more prominent role in mBERT’s impressive cross-lingual performance.\footnote{We will make our code publicly available.}
% %Our code is public\footnote{\href{https://github.com/...}{https://github.com/...}}.


==> LTH_Multilingual_LMs_EMNLP/2.introduction.tex <==


\section{Introduction}
\label{sec:introduction}

% Importance of pre-trained language models
% The emergence of transformer-based~\cite{vaswani2017attention} 
% Pre-trained language models with self-supervised objectives has revolutionized the field of natural language processing, setting state-of-the-art results in many downstream tasks~\cite{devlin2018bert, yang2019xlnet, liu1907roberta, radford2019language}.
% These language models are first trained on large unlabeled corpora; then, using smaller task-specific corpora, these general pre-trained models are fine-tuned to perform on the downstream task at hand.
% The pre-training step helps the model learn generic language representations leading to improved performance on downstream tasks and avoiding training a new model from scratch~\cite{radford2018improving, hewitt2019structure_prob, ian2019context_pprob, mario2018under_the_hood}.


% Emergence of multilingual pre-trained language models and mBERT
Multilingual language models~(MultiLMs) such as mBERT~\cite{devlin2018bert}, XLM~\cite{conneau2019cross}, and XLM-R~\cite{conneau2019unsupervised} %have shown promising zero-shot cross-lingual performance.
%These models, when 
are pre-trained jointly on raw data from multiple languages.% , learn patterns and representations for many languages in the corpus.
%
\input{floats/method_visualization}
%
Later, when they are fine-tuned for a task using perhaps a single high-resource language dataset, they demonstrate promising zero-shot cross-lingual performance, generalizing to the same task in different languages despite not having been fine-tuned for those languages.%, demonstrating promising zero-shot cross-lingual performance.

The facilitator of this cross-lingual transfer ability is often hypothesized to be a learned language neutrality in these models (\ie, similar linguistic phenomena across languages are represented similarly by the model). However, the source of this ability remains an open question. Certain studies have investigated mBERT~(a prominent MultiLM) 
for universal language-neutral components that would facilitate cross-lingual transfer~\cite{libovic2019how, pires2019multilingual, libovicky2020language}. Meanwhile, other studies claim mBERT is not language-neutral as it partitions its multilingual semantic space into separate language-specific subspaces~\cite{singh2019bert, choenni2020does, wu2019beto}.
However, most of these prior works analyze the language neutrality of MultiLMs by probing their output contextual representations.

%\citep{singh2019bert, choenni2020does, wu2019beto, libovic2019how, pires2019multilingual, libovicky2020language}. \antoine{I rephrased the previous sentence, but is this true?}\negar{Yes, except Benjamin's paper, the rest of teh papers I reviewed only analyzed the contextual representations } \antoine{okay, sounds good, though if these are all the same citations as before, we can actually probably ignore them}

% The language neutrality of these models (\ie, similar linguistic phenomena across languages are represented similarly by the model) is often hypothesized to be the main facilitator of this cross-lingual transfer ability. However, the source of this ability remains an open questions. Several studies have investigated mBERT for universal language-neutral components that could facilitate cross-lingual transfer~\cite{libovic2019how, pires2019multilingual, libovicky2020language}.
% %Multilingual BERT~(mBERT; \citealp{devlin2018bert}), one of the most widely used multilingual pre-trained models, exhibits such impressive transferability. \antoine{}
% % The exact reason for mBERT’s multilinguality is – to the best of our knowledge – still debated. 
% % mBERT is trained on the Wikipedia pages of 104 languages with a shared word piece vocabulary using masked language modeling~(MLM) and next-sentence prediction~(NSP) objectives.
% %
% % What the problem is and Previous research on language neutrality of mBERT 
% % The importance of multilingual representations and the impressive cross-lingual transfer performance of mBERT have resulted in a rich body of literature focusing on understanding the nature of mBERT representations.
% % \negar{Add language neutrality definition here}
% % Although mBERT has shown impressive transferability across languages~\cite{wu2019beto, wang2019cross}, the source of this success is still debatable.
% % the effect of its language neutrality on the performance is still debated.
% %it is still unclear to what extent its performance is related to the language neutrality of the underlying language model.
% Meanwhile, other studies claim that mBERT may not be language-neutral as it partitions its multilingual semantic space into separate language-specific subspaces~\cite{singh2019bert, choenni2020does, wu2019beto}.
% % Contrary to these studies, other efforts have claimed that mBERT also has a universal language-neutral component facilitating cross-lingual transfer~\cite{libovic2019how, pires2019multilingual, libovicky2020language}.
% % There exist several studies claiming that mBERT is not an interlingua,
% % partitioning its multilingual semantic space into separate language-specific
% % subspaces~\cite{singh2019bert, choenni2020does, wu2019beto}.
% % Contrary to these studies, the idea that in addition to the language-specific components,
% % mBERT also has a universal language-neutral component facilitating cross-lingual
% % transfer learning is also advocated~\cite{pires2019multilingual, libovicky2020language}.


% Our approach
% However, most of these prior works analyze the language neutrality of multilingual language models by probing their output contextual representations \citep{XXX}. \antoine{I rephrased the previous sentence, but is this true?}
% In this paper, we instead conceptualize language-neutrality in terms of the parameters of a model. Specifically, we hypothesize that shared parameters across different language-encoding sub-networks within multilingual language models would indicate that a multilingual model contained language-neutral representations. \antoine{too long} %Our hypothesis is that the language neutrality of multilingual language models can be exposed by comparing their learned sub-networks when they are pruned for different languages and tasks. \antoine{rephrase previous sentence -- we're being vague when we should just say the conclusion}.
% Using the lottery ticket hypothesis~\cite{frankle2018lottery}, 
% %from the neural network pruning literature to
% %The lottery ticket hypothesis
% which shows that sparse sub-networks of neural networks can be extracted and re-trained to reach the original network's accuracy (\ie, winning tickets), we discover language-specific sub-networks of different tasks and evaluate their transfer on other tasks.

% However, most of these prior works analyze the language neutrality of multilingual language models by probing their output contextual representations \citep{XXX}. \antoine{I rephrased the previous sentence, but is this true?}
In this paper, language-neutrality is instead conceptualized in terms of the parameters of MultiLMs. We hypothesize that a multilingual model with language-neutral representations would have learned different languages using the same subset of parameters in its network structure. %\antoine{rewrite previous sentence}. % subset shared parameters across different language-encoding sub-networks within multilingual language models would indicate that a multilingual model contained language-neutral representations. 
% By identifying sub-networks in multilingual language models that encode particular languages, confirming their overlap, and evaluating their transfer learning capability on other languages, we demonstrate that multilingual models learn language-neutral joint representations of multiple languages.
Sub-networks in MultiLMs that overlap across languages, and transfer well when re-trained on other languages from the pre-training corpus, would indicate that the model is comprised of language-neutral representations that jointly encode multiple languages.
%
% Using the lottery ticket hypothesis~\cite{frankle2018lottery}, 
%from the neural network pruning literature to
%The lottery ticket hypothesis
%which shows that sparse sub-networks of neural networks can be extracted and re-trained to reach the original network's accuracy, 
% we discover language-specific sub-networks in different multilingual language models and evaluate their transfer on other tasks.
%
To demonstrate this effect, we extract sub-networks from MultiLMs by pruning them for individual languages and task pairs using iterative magnitude pruning~\citep{frankle2018lottery}~(Figure~\ref{fig:methodology_step1}). 
%lottery ticket hypothesis \citep{frankle2018lottery}. 
Then, %for the same tasks, we compute the overlap of the sub-networks for different language pairs, and 
we evaluate the cross-lingual transfer of sub-networks by re-initializing to the unpruned parameters of the original MultiLM, and re-training on task data for different languages~(Figure~\ref{fig:methodology_step2}). %\antoine{previous too long}. %through one-to-one comparisons, we show that mBERT indeed includes two separate language-neutral and language-specific components.
% We also show that mBERT's language-neutral component is the main contributor to its impressive cross-lingual performance and that mBERT maps semantically-similar data points across languages close to each other.

Our results on three tasks, namely masked language modeling, named entity recognition~\citep{pan2017cross}, and natural language inference~\citep{conneau2018xnli}, show high absolute parameter overlap among sub-networks discovered for different languages and effective cross-lingual transfer between languages on the same task (even outperforming the original multilingual model for certain low-resource languages). %, perhaps due to high cross-linguistic similarity with those languages used to identify the sub-network.
However, cross-lingual sub-network transfer deteriorates as we increase the sparsity level of the sub-networks, suggesting that language-neutral components of the MultiLMs are pruned in favor of retaining necessary language- and task-specific components for the language-task pair used to discover the sub-network.

% Our main contributions are as follows:
% Using iterative magnitude pruning, we find winning tickets for masked language modeling, named entity recognition, and natural language inference tasks for multiple languages, and show that the performance of transferred sub-networks across various languages and tasks is within $\sim$4\% of the non-pruned model.

% We conclude that mBERT contains both language-specific and language-neutral components, with the latter playing a more significant role in mBERT’s impressive cross-lingual transfer performance.

% \antoine{rewrite}
% Procedurally, we first extract sub-networks from multilingual language models by pruning them for various languages and tasks. Then, through one-to-one comparisons, we show that mBERT indeed includes two separate language-neutral and language-specific components.
% We also show that mBERT's language-neutral component is the main contributor to its impressive cross-lingual performance and that mBERT maps semantically-similar data points across languages close to each other.
% Moreover, we show that well-chosen winning tickets can even outperform mBERT for low-resource languages.

% Our main contributions are as follows:
% Using iterative magnitude pruning, we find winning tickets for masked language modeling, named entity recognition, and natural language inference tasks for multiple languages, and show that the performance of transferred sub-networks across various languages and tasks is within $\sim$4\% of the non-pruned model.
% We conclude that mBERT contains both language-specific and language-neutral components, with the latter playing a more significant role in mBERT’s impressive cross-lingual transfer performance.
% Using singular vector canonical correlation analysis~(SVCCA), we show that mBERT represents semantically similar data points close to each other by learning a shared interlingual space.

% \begin{itemize}[noitemsep,topsep=0pt]
% 	\item Using iterative magnitude pruning, we find winning tickets for masked language modeling, named entity recognition, and natural language inference tasks for multiple languages, and show that the performance of transferred sub-networks across various languages and tasks is within $\sim$4\% of the non-pruned model.
	
% 	\item Using singular vector canonical correlation analysis~(SVCCA), we show that mBERT represents semantically similar data points close to each other by learning a shared interlingual space.
	
% 	\item We conclude that mBERT contains both language-specific and language-neutral components, with the latter playing a more significant role in mBERT’s impressive cross-lingual transfer performance.
% \end{itemize}

% The rest of the paper is organized as follows:
% Section~\ref{sec:related_work} provides an overview of the necessary background, related work, and the motivation of our work.
% In Section~\ref{sec:experimental_setup}, we detail our experimental settings and the techniques we use in our analysis.
% Next, we present and discuss our results in Section~\ref{sec:results}, and we conclude in Section~\ref{sec:conclusion}.


==> LTH_Multilingual_LMs_EMNLP/3.related_work.tex <==
\section{Background \& Motivation}
\label{sec:related_work}

\paragraph{Multilingual Language Models.}
% \paragraph{Multilingual BERT~(mBERT)}

% Introducing mBERT & highlighting its impressive performance
Multilingual language models~(MultiLMs) such as mBERT~\cite{devlin2018bert}, XLM~\cite{conneau2019cross}, and XLM-R~\cite{conneau2019unsupervised} have achieved state of the art results in cross-lingual understanding tasks by jointly pre-training Transformer models~\cite{vaswani2017attention} on many languages.
Specifically, mBERT has shown effective cross-lingual transfer for many tasks, including named entity recognition~\cite{pires2019multilingual, wu2019beto}, cross-lingual natural language inference~\cite{conneau2018xnli, junjie2021xtreme}, and question answering~\cite{patrick20QA}.

% The reason for mBERT's performance is not well-understood.
% Introducing previous work analyzing mBERT based on different masked language modeling pretraining regimes
Due to these impressive cross-lingual transfer results, many recent works investigate the source of this capacity.
One line of study investigates the effect of different pre-training settings (\eg, shared vocabulary, shared parameters, joint multilingual pre-training, etc.) on cross-lingual transfer \citep{wang2019cross, artetxe2020cross, conneau2020emerging}.
% Prior work has shown that shared vocabulary, shared softmax parameters, domain similarity, and joint multilingual training have a negligible effect on mBERT's cross-lingual transfer, while the depth of the network is an integral part of it~\cite{wang2019cross, artetxe2020cross, conneau2020emerging}.
% Moreover, these works demonstrated that parameter sharing plays an essential role in learning cross-lingual representation~\cite{conneau2020emerging}.
% In particular, mBERT exploits common structures across languages by aligning their representations, leading to an efficient use of limited parameters~\cite{dufter2020identify}.
%
% Previous work on the role of language neurality of mBERT on its performance
Other works explore how learned multilingual representations are partitioned into language-specific subspaces \citep{singh2019bert, wu2019beto, choenni2020does}. % mBERT's language neutrality and its connection to cross-transfer performance.
%Several studies claim that mBERT is not an interlingua as it partitions its multilingual semantic space into separate
%language-specific subspaces~\cite{singh2019bert, choenni2020does, wu2019beto}.
%
In contrast to these works, our study explores the existence of language-neutral \textit{parameters} in MultiLMs. 
Using iterative magnitude pruning, we extract pruned sub-networks from multilingual LMs for various tasks and languages, and investigate to what extent these sub-networks are similar by transferring them across languages.


\paragraph{Analysis of Multilingual Representations.}
% \paragraph{mBERT Analysis}
% \label{sec:cca_representation}

Prior work has demonstrated the lack of language neutrality in mBERT by comparing the similarity of mBERT's encodings for semantically-similar sentences across multiple languages~\cite{singh2019bert}, concluding that mBERT partitions the representation space among languages rather than using a shared, interlingual space.\footnote{In Appendix~\ref{sec:cca_representation}, we discuss how the choice of the similarity metric can affect the results of such analysis.} 
In opposition, other efforts show that mBERT learns language-neutral representation space that facilitates cross-lingual transfer~\cite{pires2019multilingual, libovic2019how, libovicky2020language}.
These findings have led to attempts to disentangle the language-specific and language-neutral components of mBERT to improve its performance~\cite{libovic2019how, libovicky2020language, Zirui2020negativeinterference, gonen2021greek, zhao2021inducing, zehui2021subnetMMT}.
The language-neutral component itself can be viewed as the stacking of two sub-networks: a multilingual encoder followed by a task-specific language-agnostic predictor~\cite{muller2021firstalign}.
% \negar{Language-specific sub-networks are also used to improve the performance of multilingual neural machine translation~\cite{zehui2021subnetMMT}.}
% The language-specific components are also considered as a potential cause of negative interference in multilingual language models~\cite{Zirui2020negativeinterference}.

In this work, we discover language-neutral components in the parameters of MultiLMs by pruning them for different language-task pairs.
% We use the lottery ticket hypothesis~\cite{frankle2018lottery} to analyze the sub-networks obtained by pruning mBERT for various languages and tasks.
By transferring sub-networks across languages, we investigate to what extent these sub-networks are language-neutral.
% \antoine{need a stronger contrastive statement}

\paragraph{Lottery Ticket Hypothesis.}

% The lottery ticket hypothesis definition
The lottery ticket hypothesis~(LTH) shows that dense, randomly-initialized neural networks contain small, sparse sub-networks~(\ie, winning tickets) capable of being trained in isolation to reach the accuracy of the original network~\cite{frankle2018lottery}.
% Therefore, smaller, carefully chosen networks can be trained from scratch to reach the same accuracy as the original network.
This phenomenon has been observed in multiple applications, including computer vision \citep{morcos2019oneticket, frankle2020linear} and natural language processing \cite{gale2019state, yu2019playing}.

% LTH is validated in BERT for several downs-stream tasks and results on the sub-nets transferability
In particular, the lottery ticket hypothesis has previously been applied to the BERT model \citep{devlin2018bert} using the GLUE benchmark~\cite{wang2019glue, prasanna2020allwinning, chen2020lottery}.
% demonstrating that even randomly selected sub-networks can perform as well as the winning tickets~\cite{prasanna2020allwinning}.
% \antoine{does this validate LTH if randomly selected subnetworks do as well at WTs ?}
% \negar{I should remove this sentence as it's related to structured pruning and not IMP. Not relevant to our analysis.}
Importantly, \citet{chen2020lottery} show that sub-networks found using the masked language modeling task can transfer to other tasks. 
In the context of multilingual language models, \citep{ansell2022composable} propose a sparse LTH-based fine-tuning method to benefit from both modular and expressive fine-tuning approaches. % while maintaining accuracy
% the transferability of winning tickets across downstream tasks has been studied in BERT, showing that sub-networks found using the masked language modeling task are universal and transfer to other tasks while maintaining accuracy~. 
In this work, we specifically use the lottery ticket hypothesis to examine the possibility of transferring winning tickets across languages, thereby disentangling whether language-neutral and language-specific components of mBERT emerge in winning tickets of different languages.

==> LTH_Multilingual_LMs_EMNLP/4.experimental_setup.tex <==
\section{Methodology}
\label{sec:methodology}
% \antoine{Few-sentence summary of what will be discussed in this section. Highlight motivation and hint at approach}
In this section, we define sub-networks (\ie, winning tickets in the LTH) and identify our approach to discovering them through a pruning algorithm derived from the lottery ticket hypothesis.

% \subsection{Sub-networks}
\paragraph{Sub-networks.}
For any network $f(x;\theta)$ with initial parameters $\theta$, we define a sub-network for $f$ as $f(x; m \odot \theta)$ where $m \in \{0, 1\}^{|\theta|}$ is a binary mask on its parameters and $\odot$ is the element-wise product. % such that its initialization is $m \odot \theta_0$ where .
The mask $m$ sets many of the parameters of the original network to zero, which prunes edges in the computation graph and yields a sub-network of the original network.

\paragraph{Winning ticket.}
When training network $f(x;\theta)$ on a task, $f$ reaches maximum evaluation performance $a$ at iteration $i$.
Similarly, when training sub-network $f(x; m \odot \theta)$ on the same task, $f$ reaches maximum evaluation performance $a^\prime$ at iteration $i^\prime$. A sub-network $f(x; m \odot \theta)$ is a winning ticket $f^*(x; m \odot \theta)$ if it achieves similar or better performance than the original network: $a - a' \leq \epsilon$ when $i^\prime \leq i$ (we set $\epsilon$ to be one standard deviation of  performance of the original mBERT model). 
% \antoine{we should use consistent notation. Later, in the results we use $p$ to refer to performance while in this section, $a$ is performance and $p$ is pruning ratios.}


\paragraph{Identifying winning tickets.}
As shown in Algorithm~\ref{alg:mip}, we use unstructured magnitude iterative pruning~\cite{han2015learning} to discover winning tickets.
In this approach, an original model is repeatedly trained on a task over multiple rounds $r$, and a subset of its parameters is pruned in each round until a desired sparsity level $s$ is reached~\cite{frankle2018lottery, chen2020lottery}.
% Using iterative pruning, we iteratively train, prune, and reset the network 
More specifically, in each round $r$ of training, the model is trained to its peak performance on the task.
Then we prune $p\%$ of the original parameters with the lowest magnitudes.
% Then, we prune $\frac{1}{p-r}$ of the remaining parameters of the model (which is equivalent to removing $\frac{|\theta|}{p}$ weights in each round where $|\theta|$ is the number of parameters in the original network).
After pruning the subset of the weights in a round $r$, the remaining weights are reset to their original pre-trained initialization, and the model is re-trained on the same dataset again. We set the iterative pruning rate $p=10$ in all experiments (e.g., five rounds to reach $s=50\%$ sparsity). To evaluate whether a sub-network is a winning ticket for a task, we check the network's task-specific performance once it has reached the desired sparsity level $s$.
Figure~\ref{fig:method_visualization} shows an overview of our approach.

\input{floats/imp_algorithm}

% \input{tables/all_tasks_winning_ticket}
\input{floats/sparsity_performance}
% \input{floats/sparsity_overlap}


\section{Experimental Setup}
\label{sec:experimental_setup}
\subsection{Model}

In our experiments, we use the cased version of multilingual BERT (mBERT; \citealp{devlin2018bert}).\footnote{\href{https://huggingface.co/bert-base-multilingual-cased}{https://huggingface.co/bert-base-multilingual-cased}}
This model is a 12-layer transformer with around 110M parameters. It is pre-trained using the masked language modeling and next sentence prediction training objectives on the Wikipedia dumps for 104 languages. A shared Wordpiece \citep{wu2016wordpiece} vocabulary of size 110k is initialized for these 104 languages.
% Moreover, for a sub-set of our experiments we use the base mT5 model (mT5-Base; \citealp{xue2021MT5}).\footnote{\href{https://huggingface.co/google/mt5-base}{https://huggingface.co/google/mt5-base}}
% This model is a multilingual text-to-text transformer trained on a multilingual variant of the C4 dataset (mC4; \citealp{raffel2020C4}) covering 101 languages.
% This 12-layer model has 580 million parameters. \antoine{I agree with Remi's comment. Maybe you can just move this to the part of the paper where you do the mT5 experiment.}

\subsection{Tasks \& Datasets}

We perform our experiments on three different NLP tasks.
We have chosen typologically diverse languages covering different language families: Germanic, Romance, Indo-Aryan, and Semitic, and including both high- and low-resource languages from the NLP perspective. 
These languages are including English~(en), French~(fr), German~(de), Chinese~(zh), Russian~(ru), Spanish~(es), Farsi~(fa), Urdu~(ur), Arabic~(ar), Hindi~(hi), and Swahili~(sw).

\paragraph{Masked Language Modeling (MLM).} For this task, we use 512-token sequences from Wikipedia in each language as the training data.
% Our study is conducted for English (en), French (fr), German (de), Chinese (zh), Russian (ru), and Spanish (es). 
    
\paragraph{Named Entity Recognition (NER).} We use WikiAnn~\cite{pan2017cross}, a multilingual named entity recognition and linking dataset built on Wikipedia articles for 282 languages\footnote{\href{https://huggingface.co/datasets/wikiann}{https://huggingface.co/datasets/wikiann}}.
Swahili~(sw) is not included in this dataset, and Hindi~(hi) has a small data size, so these two languages are excluded from the NER experiments.
% We study the English (en), French (fr), Farsi (fa), Chinese (zh), Urdu (ur), Arabic (ar), and German (de) datasets for this task.
    
\paragraph{Natural Language Inference~(NLI).} We use the cross-lingual natural language inference (XNLI) dataset~\cite{conneau2018xnli}. This dataset includes a subset of examples from MNLI~\cite{N18-1101} translated into 14 languages\footnote{\href{https://huggingface.co/datasets/xnli}{https://huggingface.co/datasets/xnli}}.
Farsi is not included in this dataset.% License: CC BY-NC 4.0
% We used the English (en), French (fr), Arabic (ar), Chinese (zh), Hindi (hi), Urdu (ur), and Swahili (sw) datasets for our experiments.

\subsection{Training Details}

We tune hyperparameters and select evaluation metrics for each task based on prior work~\cite{chen2020lottery}\footnote{\href{https://github.com/VITA-Group/BERT-Tickets}{https://github.com/VITA-Group/BERT-Tickets}}.
All results are reported on the development sets of these datasets and are the average of three runs using different random seeds.
We use the same number of training and evaluation examples for all languages of a task.
Table~\ref{table:train_details} in the appendix reports pre-training and fine-tuning details. 
Computational details are reported in Appendix~\ref{sec:computation}.
% MLM and NER tasks and one run for the XNLI task due to computation complexity.



% \input{tables/experiment_setup}




==> LTH_Multilingual_LMs_EMNLP/5.results.tex <==
% \input{tables/all_tasks_winning_ticket}

\input{floats/sparsity_overlap}

\section{Experimental Results}
\label{sec:results}

In this section, we report our evaluations to study the presence of language-neutral sub-networks in multilingual language models.
First, we validate the lottery ticket hypothesis for the mBERT model for various languages and tasks.
Then, we compare the winning tickets for different languages by analyzing their parameter overlap and cross-lingual performance.
% First, we validate the lottery ticket hypothesis for the mBERT model for various languages and tasks by demonstrating the existence of sub-networks that perform as strongly (or better) than the original mBERT model on these tasks.
% Then, we evaluate the cross-lingual performance of winning tickets for particular languages and tasks, demonstrating that sub-networks discovered for particular task-language pairs can generalize to other languages (though they are not as successful for task transfer).
% We further assess the similarity of discovered sub-networks by computing their parameter overlap. %and examine to what degree language-neutral and language-specific patterns emerge in these sub-networks by computing their overlap.  % and comparing their performance in a zero-shot setting
Finally, to further assess the similarity of the winning tickets in a zero-shot setting, we evaluate their performance in a sentence retrieval task. 

\paragraph{Existence of Winning Tickets.}
% \label{sub:winning_tickets_existence}

To discover winning tickets for each task-language pair, we run Algorithm~\ref{alg:mip} to identify sub-networks at various sparsity levels. Then, we train the pruned sub-networks on the same task and language to identify whether it qualifies as a winning ticket, $f^*(x, m \odot \theta)$.
%Table~\ref{table:all_in_result} exhibits our results for the MLM, XNLI, and NER tasks on the languages selected in Section~\ref{sec:experimental_setup}. 

 %Furthermore, we confirm that these sub-networks perform better than randomly sampled sub-network at the same sparsity level $s$.% rather than using the iterative magnitude pruning to search for better performing sub-networks.
%
% For the MLM task, the highest sparsity level for which we could find winning tickets is 50\%.
% For the XNLI task, we find winning tickets at the sparsity level of 50\% for all languages except Urdu, which has a winning ticket at 30\% sparsity.
% The performance gap between the pruned sub-network of Urdu and mBERT on the same sparsity level is around 1\%.
% Finally, for the NER task, we find winning tickets for all the languages: at the sparsity level of 50\% for Chinese, Arabic, and German, and at sparsity of 60\% for the rest of the languages.
%
In Figure~\ref{fig:sparsity_performance}, we report the performance of pruned sub-networks for each task-language pair at different sparsity levels between 0 and 90\%. Winning tickets are found for each language and task at multiple sparsity levels, though as these sub-networks get sparser, they no longer satisfy the winning ticket criterion (performance must be within 1 standard deviation of the full mBERT performance). However, they still often perform within 10\% of their winning ticket performance. Interestingly, we find that the performance drop at higher sparsity levels is greater for the MLM and NER tasks than for XNLI, highlighting the importance of evaluating on tasks that induce diverse behavior in sparse models. %\antoine{why is this interesting?} \negar{We wanted to point out the different behavior these tasks have, but I think it doesn't add anything and we should remove it }
%Appendix~\ref{sec:more_result_on_lth}.

% \input{tables/MLM_winning_tickets}
% \input{tables/XNLI_winning_tickets}
% \input{tables/NER_winning_tickets}

% \subsection{Discovering Language-neutral Sub-networks}
% \label{sec:cross-ling}
\paragraph{Absolute Sub-network Overlap.}

Given that we can discover suitable winning tickets for every language and task, we now assess the similarity of the discovered sub-networks by comparing their parameter overlap.
Sub-network pairs (or larger groups) with higher overlap will be more likely to correspond to language-neutral representations in the original mBERT model. 
To measure parameter overlap between discovered sub-networks for different task-language pairs, we compute the Jaccard similarity between masks~($m_i$, $m_j$) from two sub-networks~$\big(\frac{m_i \cap m_j}{m_i \cup m_j}\big)$.
In Figure~\ref{fig:sparsity_overlap}, we report the parameter overlap across mBERT's layers for different language pairs across each of the tasks. These results are for sub-networks at $50\%$ sparsity, so we note that the expected Jaccard similarity of two randomly sampled $s$=$50\%$ sparse sub-networks would be $33\%$.

We find that the NER task generally discovers sub-networks with much more overlap across languages, followed by XNLI and MLM. Both NER and XNLI exhibit increasingly overlapping sub-networks at higher layers, while sub-networks discovered for the MLM task increase in overlap up until the middle layers and then drop again. This phenomenon is perhaps partly explained by the upper layers being more task-focused \citep{merchant2020whathappens}. For the MLM task, the model must predict language-specific tokens as the task. While we do not prune the task heads as part of our algorithm, the upper layers of mBERT may still need to be specialized to particular languages to predict their unique vocabularies\footnote{Further analysis of these MLM results is in Appendix~\ref{sec:subnet_overlap}.}.

% The overlap across sub-networks trained for the same task or language across multiple runs
As a comparison, we establish an upper bound on the expected overlap between languages, by computing the overlap of sub-networks for the same language~(pruned using different random seeds).
The average overlap of sub-networks across multiple runs is 98.66, 92.23, and 92.23 for the NER, XNLI, and MLM tasks, respectively.
In all three tasks, the overlaps across runs are much higher than the mask overlap across languages.

\paragraph{Cross-lingual Transfer of Winning Tickets.}
We now evaluate the transfer of winning tickets across languages for a given task. %In particular, we check whether the winning ticket for a particular language and task is also a winning ticket for others languages for the same task.
Using the discovered sub-networks for each task-language pair (set at a sparsity level of $50\%$ to maintain consistency across languages), we train these sub-networks on the other task-language pairs for the same task and compare their performance against the original sub-network trained on identical data (\ie, $a(s, t)$ vs $a(t, t)$\footnote{$a$ stands for the performance metric of the model as mentioned in Section~\ref{sec:methodology}.} where $s$ stands for the \textit{source} language and $t$ stands for the \textit{target} language).
% For this set of experiments, we use sub-networks with 50\% sparsity.
%
% Next, we evaluate the performance of newly trained models on the same task and language they were trained on and compare them against mBERT's performance for the source language.
If a transferred sub-network's performance on the \textit{target} language is within one standard deviation of the \textit{target} language sub-network's performance, we identify it as a successful transfer, indicating that this winning ticket is more language-neutral than language-specific, as its original parameters are adaptable for different languages. 
%\antoine{It might be good to write this out as an algorithm or use some notation. It's very intuitive, but it ends up sounding jumbled }\negar{something like $|p(s, t) - p(t, t)| < \epsilon$ you mean? yes, except I'm not sure that's the actual condition ? --  we should use the winning ticket definition here. if the transferred performance is in one std of the original sub-network. because in the following we talk about a winning ticket in a language being a winning ticket for other languages.} \antoine{Does the winning ticket condition have the absolute value? Seems like it was just $p(s,t) - p(t,t) < \epsilon$} \negar{you're right, it doesn't have the absolute value. I've also added it without absolute value in the following text.}

\input{floats/cross_language_transfer}

Figure~\ref{fig:MLM_transfer} shows the transfer performance (\ie, the performance drop or gain of the sub-network when trained on the \textit{target} language compared to when trained on the \textit{source} language) of MLM winning tickets. %(sub-networks discovered using the \textit{source} language; $p(s, t) - p(t, t)$).
% Each cell indicates the difference between the transferred sub-network performance and source language sub-network's performance.
For this task, none of the winning tickets for source languages are winning tickets for other languages, meaning that the sub-networks do not achieve similar perplexity as to the \textit{target} sub-networks when transferred to the target tasks. %\antoine{is this a comparison to full model? or to subnetwork trained on source language?} \negar{comparison to source language subnetwork, but to be a winning ticket it needs to meet the full model performance, but it's better to mention the source subnetwork}
However, the perplexity increase is relatively limited~(within $0.2$-$0.5$ points) compared to a $50\%$ sub-network pruned randomly (rand), suggesting that these language-specific sub-networks do contain shared multi-lingual components.% representations. 

% showing that although MLM needs language-specific information to predict the missing word correctly, the language-neutral part of the sub-networks is still dominating.
A similar transfer pattern emerges for the NER task in Figure~\ref{fig:NER_transfer}.
None of the transferred sub-networks match the performance of the source language sub-network. However, the performance remains high, with most target languages maintaining 98\% of the target sub-network performance when trained on the source sub-networks (compared to when trained on a random sub-network)\footnote{We also developed additional random baselines where LTH-discovered sub-networks at 10, 20, 30, and 40\% sparsity are randomly pruned to reach a 50\% sparse sub-network. Although the performance of these baselines is higher, transferring sub-networks across languages still outperforms them.}.
%
% an F1-score of $\sim$90\% 
% It shows once again that the winning tickets contain more information on the task they are pruned on than the language the training data comes from.
% Interestingly, Chinese (zh) experiences the worst performance drop when we use sub-networks trained for other languages to transfer for this language.
Chinese~(zh) and Urdu~(ur) experience the worst performance drop when we use sub-networks trained for other languages to transfer for these two languages.
One explanation could be that Chinese NER is more challenging than other languages due to the lack of capitalization information and the challenge of word segmentation in Chinese. Consequently, Chinese may require more language-specific information that may be pruned from the sub-networks of other languages.
The relatively low transfer performance for Urdu may be more empirical. Urdu's sub-network at 50\% sparsity has a high performance, outperforming mBERT by 1.2 points, making it a strong baseline.
% We note that the highest sparsity level in which we found a winning ticket for Urdu is 60\%.
% \antoine{We need to motivate why we note this or take it out.}
% Hence, Chinese NER requires more language-specific information that is absent in other sub-networks.

The results for the XNLI task (depicted in Figure~\ref{fig:XNLI_transfer}) exhibit a different pattern.
For XNLI, the sub-networks found for a language often perform well for other languages, hinting at significant language-neutral components in these sub-networks. At times, these transferred sub-networks even exceed the performance of the source language sub-networks.
For example, the French and English winning tickets are also winning tickets for all other languages we examined.
The Spanish, Russian, and German sub-networks also transfer well to most other languages.
However, the transfer performance of Urdu\footnote{For XNLI, the sparsest Urdu winning ticket was at $s=30\%$. For consistency, we used a 50\% sparse sub-network for Urdu in these experiments, but the 30\% sparse sub-network does not transfer well to other languages either.} and Swahili sub-networks are worse than other languages, possibly because these two languages were under-represented during mBERT's pre-training, and so contributed less to the model's final parameters compared to other languages\footnote{Urdu and Swahili have less than 200k Wikipedia articles while the rest are on the scale of millions of articles:  \href{https://meta.wikimedia.org/wiki/List_of_Wikipedias}{https://meta.wikimedia.org/wiki/List\_of\_Wikipedias}}.
% Moreover, the NLI task requires a semantic interpretation of the text, which needs a semantically rich representation that can only be obtained from large corpora.
%
% The high transfer performance of XNLI sub-networks is another indication of the significant role of the language-neutral component of these sub-networks.
We also note that Arabic's winning ticket outperforms mBERT by $\sim$1.5 points for Swahili and Urdu. 
As both Urdu and Swahili have been historically influenced by Arabic~\cite{spear2000early, versteegh2014arabic}, they may benefit from Arabic being a high resource language in the pre-training corpus.

\input{floats/mt5_transfer_results}


Interestingly, the parameter overlaps of all the language pairs do not always predict their cross-lingual transfer performance. 
For MLM, the lower relative degree of sub-network overlap between languages does align with the observed performance drop when transferring winning tickets between languages~(Figure~\ref{fig:MLM_transfer}). Similarly, an increased overlap is observed among XNLI sub-networks, corresponding to improved transfer performance between languages. When looking at the NER sub-networks, however, which have the highest pairwise overlap, we do not observe successful transfer results~(Figure~\ref{fig:NER_transfer}). We conjecture that transfer for NER may require specialized knowledge about the entities likely to be discussed in a particular language (\eg, Chinese Wikipedia articles in the NER dataset may contain more information about Chinese public and historical figures). Consequently, even if a high overlap is observed, the non-overlapping parameters in these sub-networks are crucial for successful task performance\footnote{Further analysis is in Appendix~\ref{sec:cross-task}.}.

% The absolute performance values of all three tasks are provided in Appendix~\ref{sec:more_result_on_lth}.
To investigate to what extent these observations generalize to other models, we repeat the same experiments for the mT5 model~\citep{xue2021MT5}.\footnote{\href{https://huggingface.co/google/mt5-base}{https://huggingface.co/google/mt5-base}}
This model is a multilingual text-to-text transformer with 12 layers and 580 million parameters and is trained on a multilingual variant of the C4 dataset~(mC4; \citealp{raffel2020C4}) covering 101 languages.
We formulate the XNLI task into a text-to-text format similar to the mT5 paper by generating the label text from the concatenation of the premise and hypothesis.
%We pruned the encoder and decoder separately.
Figure~\ref{fig:mt5_results} shows the cross-lingual transfer performance for the XNLI task at 50\% sparsity level.\footnote{We note that winning tickets for these languages are not found for this sparsity level, but chose to maintain consistency with the mBERT experiments.}
For most cases, the transfer performance drop is relatively small, and, as with mBERT, similar languages such as English, Spanish, French, and German transfer well to most of the other languages, suggesting that language-neutral parameters are a common phenomenon in different MultiLMs.
%This observation is yet another evidence of the existence of language-neutral components in the MultiLMs that facilitate the cross-lingual transfer.

\input{floats/avg_performance_drop}


% \input{floats/mt5_transfer_results}

\paragraph{Impact of Sub-network Density.} To investigate the effect of sparsity on the retainment of language-neutral components, we compare the cross-lingual transferability of mBERT sub-networks at 50\% and 80\% sparsity levels. 
Figure~\ref{fig:avg_perf_drop} shows the average of relative transfer performance drop\footnote{$\frac{1}{\vert L \vert - 1}\sum_{t \in L \setminus s} \frac{a(s, t) - a(t, t)}{a(t, t)}$ where $s$ and $t$ are source and target languages and $L$ is the set of languages for each task.} 
per language for the NER and XNLI tasks. Each bar represents an average performance drop after retraining (and evaluating) the sub-network for the source language on all the target languages, individually.
As we increase the sparsity level of a sub-network, its cross-lingual transferability degrades considerably (\ie, the \textit{relative} performance drop \textit{increases}), indicating that there were language-neutral parameters at 50\% sparsity level facilitating the cross-lingual transfer that were pruned in the 80\% sparse sub-network.
As we decrease the model's capacity by pruning more parameters, the model relies more on language- and task-specific parameters than those that may facilitate the cross-lingual transfer.
% \input{floats/avg_performance_drop}


 %The overlaps for MLM and XNLI tasks match their transfer performance (from Section~\ref{sec:cross-ling}). %cf., Figure~\ref{fig:all_transfer}).
% The NER sub-networks, however, have large overlaps while showing relatively lower transferability performance.
% We hypothesize that NER requires fewer (but specific) parameters than the other two, and only a tiny fraction of language-specific parameters is enough to specialize a sub-network for a language.

% Figure~\ref{fig:sparsity_overlap} shows the parameter overlap across mBERT's layers for each of the mentioned tasks.
% The overlap increases for the NER and the XNLI tasks as we go into deeper layers, with the highest overlap in the last layer.
% We know that fine-tuning primarily affects the top layers of the model, and these layers are more task-specific than the rest~\cite{merchant2020whathappens}.
% Hence it was expected that the last layers would be more similar across language; in other words, they are more language-neutral.
% For the MLM task, the overlap increases up to 8\textsuperscript{th} layer and then starts to decrease.
% In the top layers, MLM needs language-specific information to correctly predict the missing word. It explains why these sub-networks are more language-specific in the last layers than the middle ones.

% The overlap across sub-networks for all languages for the MLM, NER, and XNLI tasks are around 53\%, 92\%, and 75\%, respectively, while the overlap across all tasks and languages is around 51\%, which suggests that mBERT that mBERT exploits common features across tasks during the pre-training.
% We leave detailed exploration on sub-networks overlap to future work by including more downstream tasks and languages.

\input{floats/translation_accuracy}

\paragraph{Parallel Sentence Retrieval.}

% \antoine{what's the motivation? -- why did we specifically select this experiment?}
To further assess the language neutrality of mBERT, we compare the behavior of different sub-networks in a zero-shot setting where they are used as feature extractors. 
We evaluate each sub-network's sentence retrieval accuracy~\cite{pires2019multilingual} on the English-to-French translation test set from the WMT14 dataset~(3003 sentence pairs).\footnote{\href{https://huggingface.co/datasets/wmt14}{https://huggingface.co/datasets/wmt14}}
This task aims to find sentence pairs from two corpora in two different languages, where the two sentences of each pair are corresponding translations of one another. 
In these experiments, we use the parallel retrieval implementation from LASER\footnote{\href{https://github.com/facebookresearch/LASER}{https://github.com/facebookresearch/LASER}} with the margin-based scoring function from~\cite{artext2019margin}.\footnote{The definition of the function is available in Appendix~\ref{sec:scoring_func}.} 
We use the average of the token embeddings for each sentence (encoded using the sub-networks) as the retrieval inputs.
% \begin{multline*}
% \mbox{score}(x, y) = \mbox{margin}(cos(x, y), \\ \sum_{z \in \mathcal{N}_{k}(x)} \frac{cos(x, z)}{2k} + \sum_{z \in \mathcal{N}_{k}(y)} \frac{cos(y, z)}{2k})
% \end{multline*}

% \begin{multline*}
% s(x, y) = \frac{cos(x, y)}{\sum\limits_{z \in \mathcal{N}_{k}(x)} \frac{cos(x, z)}{2k} + \sum\limits_{z \in \mathcal{N}_{k}(y)} \frac{cos(y, z)}{2k}}
% \end{multline*}

% \noindent where $x$ and $y$ are two sentence representations and $\mathcal{N}_k(x)$ denotes the $k$ nearest neighbors of $x$ in the other language. 

%We use $\mbox{margin}(a, b) = a/b$ as our margin function.
% \antoine{average representations from what?}
% Figure~\ref{fig:translation_accuracy} shows the retrieval accuracy~(top-5) when using output embeddings of different layers of the sub-network as the retrieval input.

% For the XNLI task, the English (en) and French (fr) sub-networks outperform others in shallower layers, but the rest catch up in the middle layers.
% From there, German and Hindi get separated in layer 10, while the rest continue to perform similarly.
We observe that both the similarity across the sub-networks (Figure~\ref{fig:mlm_sparsity_overlap}) and the top-5 retrieval accuracy (Figure~\ref{fig:translation_accuracy}) increase as we go into the middle layers of mBERT. %\antoine{}
%However, while the 
% As this task requires a high semantic abstraction, this observation indicates that semantic abstraction occurs as we go toward the middle layers.
% \antoine{this reasoning isn't obvious, so needs to be outlined more explicitly in the running text}
% Then, at the highest layers, the task-specific parameters of the networks dominate the the rest, and the retrieval accuracy drops. \antoine{why?} \negar{ because the last layers focus more on the task they were pruned for and they're not good as multilingual feature encoders} \antoine{but then in the last layer (the one closest to the task), the performance rises again?} \negar{I think we should remove the previous sentence because I really don't know what's happening in the layers 11 and 12.}
XNLI's winning tickets perform better than the other two tasks, and some of these sub-networks even reach the same zero-shot accuracy as the full mBERT model.
One possible explanation is that both the XNLI task and parallel sentence retrieval require a richer semantic interpretation of the text. Hence, XNLI winning tickets are better sub-networks for parallel sentence retrieval as they must capture semantic knowledge to successfully complete the task. 
In the case of NER, the sub-networks of different languages perform similarly across all layers, which is unsurprising given the high amount of overlap between these sub-networks. In a zero-shot setting with no language-specific tuning for the task, these sub-networks are basically identical.
% As before, we hypothesize that language-neutral parts of these sub-networks are dominating, and the language-specific parts have a negligible effect on the captured semantic knowledge of these sub-networks. %\antoine{this seems to contrast with the results of the previous experiments, where language-specific components were necessary for task transfer, which is why there could be high overlap w/o good task transfer } \negar{ language-specific components were necessary for the NER task, but I guess just a small fraction of parameters were enough for NER. So, we have a large part of the parameters being language-neutral which is a benefit for sentence retrieval task.}.
For MLM, the sub-networks perform similarly up to the middle layers, where they begin to diverge, supporting the hypothesis that higher layers in the MLM sub-networks are dedicated toward representing the task, which is language-specific for MLM. %Regardless, the relatively high performance of these sparse subnetworks for retrieving sentences in another language supports the presence
% \antoine{why does French overall do worse? why does Spanish drop after layer 6? -- I don't have explanation for these observations.. }
% We leave detailed analysis of such behaviors for future work.

\paragraph{Multilingual Sub-networks.}
Observing the benefit of transferring sub-networks from high-resource languages to lower resource ones (\eg, Arabic to Urdu and Swahili for NER), we study the impact of combining datasets from multiple languages to discover multilingual winning tickets.
In this set of experiments, we combined English, Farsi, French, and Chinese datasets together to prune mBERT for the NER task. For parity, we use an identically-sized combined training dataset with 20,000 samples (the same as other experiments on this task), keeping only 25\% of each of each language's dataset.
Table~\ref{table:combined_datasets} shows the transfer results of the resulting sub-network at 50\% sparsity level.
For three out of five languages that we evaluated transfer performance on, the sub-network extracted using the combination of languages outperforms the sub-networks found using each training language separately. The inclusion of multiple languages in the corpus may encourage recovering more language-neutral sub-networks than discovering sub-networks using only a single language.
% This observation tells us that with the same number of training data, sometimes it is better to combine datasets from several languages than using a single language.
% Languages can benefit from multiple languages in different ways.
% For instance, in this experiment, Urdu and Arabic may benefit from Farsi being in the training data because all three share the same writing scripts.
% They can also benefit from English or French as high-resource languages that have contributed more in the pre-training phase.

\input{tables/combined_datasets}

==> LTH_Multilingual_LMs_EMNLP/6.conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

% Emergence of multilingual pre-trained language models and mBERT
% Do not know why mBERT is so good
% Our key insight is that the extent of mBERT's language neutrality can be exposed by comparing the sub-networks within mBERT obtained by pruning it for different languages and tasks.
% In this paper, we first extract sub-networks from mBERT pruned for various languages and tasks; then, through one-to-one comparisons, we show that mBERT indeed includes two separate language-neutral and language-specific components.
% We also show that mBERT's language-neutral component is the main contributor to its impressive cross-lingual performance and that mBERT maps semantically-similar data points across languages close to each other.
% Moreover, we show that well-chosen winning tickets can even outperform mBERT for low-resource languages.

While multilingual pre-trained language models %such as mBERT
have shown impressive performance across languages, the role of language neutrality in achieving such a performance is not well understood.
In this work, we analyze the language-neutrality of multilingual models by investigating the overlap between language-encoding sub-networks of these models.
Using mBERT as a foundation, we expose the extent of its language neutrality by employing the lottery ticket hypothesis and comparing the sub-networks within mBERT obtained for various languages and tasks.
We show that such sub-networks achieve high performance after being transferred across tasks and languages and are similar to one another. However, at higher levels of sparsity, this transferability evaporates. Our results suggest that multilingual language models include two separate language-neutral and language-specific components, with the former playing a more prominent role in cross-lingual transfer performance.
% We conclude that mBERT maps semantically-similar sentences across languages close to each other and that mBERT's language-neutral component plays a major role in its impressive cross-lingual performance.
% These observations are worthy of further investigation, and we aim to include more downstream tasks, languages, and network similarity metrics in our future work.

==> LTH_Multilingual_LMs_EMNLP/7.limitation.tex <==
\section*{Limitations}
In this work, we use network parameter overlap to measure similarity between sub-networks discovered for different languages.
However, while cross-lingual transfer performance coarsely tracks with sub-network overlap, these results may not hold at a fine-grained level. While high sub-network overlap is an indicator that a sub-network will effectively transfer to a target language, small relative differences in cross-lingual performance across languages do not correlate strongly with overlap. Consequently, absolute overlap may be limited as an analogue for identifying language-neutral components of multilingual models.
% So, we need to go for the metrics that measure these sub-networks similarity based on their performance on a downstream task.
Another limitation is that we only use the lottery ticket hypothesis as a method for discovering language-specific sub-networks, while other pruning and masking methods may provide complementary or competing insights.
Finally, due to computational limitations, we only apply our work to three tasks and eleven languages. While our selection is diverse, new insights may emerge from a larger cross-section.

==> LTH_Multilingual_LMs_EMNLP/floats/avg_performance_drop.tex <==
\begin{figure}
    \centering
    % \subfloat[MLM]{
    %     \label{fig:mlm_sparsity_overlap}
    %     {\includegraphics[width=0.30\textwidth]{figures/MLM_sparsity_overlap.pdf}}
    % }
    \centering
    \subfloat[NER]{
        \label{fig:ner_perf_drop}
        {\includegraphics[width=0.85\columnwidth]{figures/NER_performance_drop.pdf}}
    }
    
    \centering
    \subfloat[XNLI]{
        \label{fig:xnli_perf_drop}
        {\includegraphics[width=0.85\columnwidth]{figures/XNLI_performance_drop.pdf}}
    }
    \caption{Average cross-transfer performance drop for sub-networks with sparsity levels 50\% and 80\%. For each source language and task, the relative average is computed across the other languages and the same task.}
    \label{fig:avg_perf_drop}
    \vspace{-4mm}
\end{figure}


==> LTH_Multilingual_LMs_EMNLP/floats/cca_similarities.tex <==
\begin{figure}
    \centering
    \subfloat[PWCCA]{
         \label{fig:pwcca_xnli}
        {\includegraphics[width=0.8\columnwidth]{figures/PWCCA_scores.pdf}}
    }
    
    \subfloat[SVCCA]{
         \label{fig:svcca_xnli}
        {\includegraphics[width=0.8\columnwidth]{figures/SVCCA_scores.pdf}}
    }
    \caption{Similarity scores between CLS representations of English and five other languages using PWCCA and SVCCA.}
    \vspace{-4mm}
\end{figure}



==> LTH_Multilingual_LMs_EMNLP/floats/cross_language_transfer.tex <==
\begin{figure}
    \centering
    \subfloat[MLM]{
        \label{fig:MLM_transfer}
        {\includegraphics[width=0.86\columnwidth]{figures/MLM_transfer.pdf}}
    }
    
    \subfloat[NER]{
        \label{fig:NER_transfer}
        {\includegraphics[width=0.86\columnwidth]{figures/NER_transfer.pdf}}
    }
    
    \subfloat[XNLI]{
        \label{fig:XNLI_transfer}
        {\includegraphics[width=0.86\columnwidth]{figures/XNLI_transfer.pdf}}
    }
    
    
    \caption{The performance difference of transferring winning tickets across languages~(50\% sparsity).
    Each row indicates the source language and each column indicates a target language.
    Each cell shows the difference in performance between the transferred sub-network and the sub-network discovered from training directly on the target language.
    We also report the performance drop of a random sub-network (\textbf{rand}) compared to the language sub-network.
    Blue and red colors indicate performance losses and gains respectively.
    %Perplexity, F1, and accuracy are the performance metrics for MLM, NER, and XNLI, respectively.
    }
    \label{fig:all_transfer}
    \vspace{-4mm}
\end{figure}

==> LTH_Multilingual_LMs_EMNLP/floats/cross_task_transfer.tex <==
\begin{figure}
     \centering
    \subfloat[Target task: MLM ]{
        \label{fig:mlm_cross_task}
        {\includegraphics[width=0.9\columnwidth]{figures/cross-MLM_transfer}}
    }
    
    \centering
    \subfloat[Target task: NER ]{
        \label{fig:ner_cross_task}
        {\includegraphics[width=0.9\columnwidth]{figures/cross-NER_transfer}}
    }
    
    \centering
    \subfloat[Target task: XNLI]{
        \label{fig:xnli_cross_task}
        {\includegraphics[width=0.9\columnwidth]{figures/cross-XNLI_transfer}}
    }
    
    \caption{The performance of transferring winning tickets between tasks~(50\% sparsity).
        Each cell shows the difference in performance between the transferred sub-network and the performance of the sub-network discovered for the target task. %\antoine{confusing caption}
        }
        \label{fig:cross_task_transfer}
    \vspace{-4mm}
\end{figure}

==> LTH_Multilingual_LMs_EMNLP/floats/imp_algorithm.tex <==
\begin{algorithm}[t]
\footnotesize
\caption{Iterative magnitude pruning to reach sparsity level $s$.}
\label{alg:mip}

\begin{algorithmic}
\State Start with mBERT pre-trained weights $\theta_0$
\State Set $p \gets 10$ and $n \gets \frac{s}{p}$
\For{$r \gets 0$ to $n-1$}                 
    \State Train network for $i$ iterations, arriving at parameters $\theta_i$
    \State Prune $p\%$ of the parameters in $\theta_0$
    % \State Prune $\frac{1}{p-r}$ of the parameters in $\theta_i$
    \State Reset the remaining parameters to their values in $\theta_0$
\EndFor
% \Repeat 
% \State Train the network for $i$ iterations, arriving at parameters $\theta_i$
% \State Prune $10\%$ of the parameters in $\theta_i$
% \State Reset the remaining parameters to their values in $\theta_0$
% \Until{meets the sparsity level $s$}
\State Return the resulted pruned network
\end{algorithmic}
\end{algorithm}

==> LTH_Multilingual_LMs_EMNLP/floats/method_visualization.tex <==
\begin{figure}[!ht]
\centering
\subfloat[Step 1: Discover sub-networks in multilingual language models that encode particular languages]{
        \label{fig:methodology_step1}
        {\includegraphics[width=0.79\columnwidth]{figures/monolingual-subnet-graph.pdf}}
    }

\vspace{-2mm}

\subfloat[Step 2: Transfer sub-networks to new languages to evaluate their language neutrality degree]{
        \label{fig:methodology_step2}
        {\includegraphics[width=0.79\columnwidth]{figures/cross-lingual-transfer-graph.pdf}}
    }
% \includegraphics[width=0.8\columnwidth]{figures/methodology_graph.pdf}
\caption{Overview of our approach.
We discover sub-networks in the original multilingual language model that are good foundations for learning various tasks and languages (a). Then, we investigate to what extent these sub-networks are similar by transferring them across other task-language pairs (b).
In this example, the \textcolor{blue}{blue} and \textcolor{red}{red} lines show sub-networks found for French and Urdu, respectively, and \textcolor{violet}{purple} connections are shared in both sub-networks. Dashed lines show the weights that are removed in the pruning phase. }
\label{fig:method_visualization}
\vspace{-6mm}
\end{figure}

==> LTH_Multilingual_LMs_EMNLP/floats/mt5_network_overlap.tex <==
\begin{figure*}
    \centering
    \subfloat[Encoder]{
        \label{fig:mt5_encoder_network_overlap}
        {\includegraphics[width=0.50\textwidth]{figures/mt5_encoder_overlap.pdf}}
    }
    \centering
    \subfloat[Decoder]{
        \label{fig:mt5_decoder_network_overlap}
        {\includegraphics[width=0.50\textwidth]{figures/mt5_decoder_overlap.pdf}}
    }
    \caption{Sparsity pattern overlap between pruned sub-networks across different layers at 50\% sparsity level for the XNLI task on the mT5 model.}
    \label{fig:mt5_network_overlap}
    \vspace{-4mm}
\end{figure*}


==> LTH_Multilingual_LMs_EMNLP/floats/mt5_transfer_results.tex <==
\begin{figure}
\centering
\includegraphics[width=0.9\columnwidth]{figures/mt5_transfer.pdf}
\caption{The performance difference of transferring
winning tickets across languages (50\% sparsity) for the XNLI task on the mT5 model.}
\vspace{-4mm}
\label{fig:mt5_results}
\end{figure}

==> LTH_Multilingual_LMs_EMNLP/floats/sparsity_overlap.tex <==
\begin{figure*}

    \centering
    \subfloat{
        {\includegraphics[width=1\textwidth]{figures/overlap_legend.png}}
    }
    
    \addtocounter{subfigure}{-1}
    
    \centering
    \subfloat[MLM]{
        \label{fig:mlm_sparsity_overlap}
        {\includegraphics[width=0.32\textwidth]{figures/MLM_overlaps.pdf}}
    }
    \centering
    \subfloat[NER]{
        \label{fig:ner_sparsity_overlap}
        {\includegraphics[width=0.32\textwidth]{figures/NER_overlaps.pdf}}
    }
    \centering
    \subfloat[XNLI]{
        \label{fig:xnli_sparsity_overlap}
        {\includegraphics[width=0.32\textwidth]{figures/XNLI_overlaps.pdf}}
    }
    \caption{Sparsity pattern overlap between pruned sub-networks across different layers at 50\% sparsity level.}
    \label{fig:sparsity_overlap}
    \vspace{-4mm}
\end{figure*}


==> LTH_Multilingual_LMs_EMNLP/floats/sparsity_performance.tex <==
\begin{figure*}
    \centering
    \subfloat{\includegraphics[width=0.55\textwidth]{figures/sparsity_plot_legend.pdf}}
    
    \addtocounter{subfigure}{-1}
    
    \centering
    \subfloat[MLM]{
        \label{fig:mlm_sparsity}
        {\includegraphics[width=0.32\textwidth]{figures/MLM_sparsity.pdf}}
    }
    \centering
    \subfloat[NER]{
        \label{fig:ner_sparsity}
        {\includegraphics[width=0.32\textwidth]{figures/NER_sparsity.pdf}}
    }
    \centering
    \subfloat[XNLI]{
        \label{fig:xnli_sparsity}
        {\includegraphics[width=0.32\textwidth]{figures/XNLI_sparsity.pdf}}
    }
    \caption{Performance of pruned sub-networks for each task-language pair at different sparsity levels}
    \label{fig:sparsity_performance}
    \vspace{-4mm}
\end{figure*}

==> LTH_Multilingual_LMs_EMNLP/floats/translation_accuracy.tex <==
\begin{figure*}
    \centering
    \subfloat{
        % \label{fig:sentence}
        {\includegraphics[width=0.75\textwidth]{figures/sentence_retrieval_legend.png}}
    }
    
    \addtocounter{subfigure}{-1}
    
     \centering
    \subfloat[MLM]{
        \label{fig:mlm_translation}
        {\includegraphics[width=0.32\textwidth]{figures/MLM_retrieval.pdf}}
    }
    \subfloat[NER]{
        \label{fig:ner_translation}
        {\includegraphics[width=0.32\textwidth]{figures/NER_retrieval.pdf}}
    }
    \subfloat[XNLI]{
        \label{fig:xnli_translation}
        {\includegraphics[width=0.32\textwidth]{figures/XNLI_retrieval.pdf}}
    }
        \caption{Parallel sentence retrieval accuracy on English-to-French translation using winning tickets.
        We use the average of the contextual embeddings of each sentence as the retrieval inputs.}
        \label{fig:translation_accuracy}
    \vspace{-4mm}
\end{figure*}

==> LTH_Multilingual_LMs_EMNLP/tables/MLM_cross_lang.tex <==
\begin{table*}[t]
% \footnotesize
  \centering
\resizebox{\textwidth}{!}{
\begin{tabular}{ l c c c c c c c c c c c}
\toprule
\textbf{Model /} & \multicolumn{11}{c}{\textbf{Target Language}} \\
% \midrule
\textbf{Sub-network}  & \textbf{ar} & \textbf{de} & \textbf{en} & \textbf{es} & \textbf{fa} & \textbf{fr} & \textbf{hi} & \textbf{ru} & \textbf{sw} & \textbf{ur} & \textbf{zh} \\
\midrule
\textbf{mBERT} & 3.5247 & 3.5143 &  4.6523 & 3.6775 & 3.8033 & 3.1151 & 2.8728 & 2.5927 & 2.5001 &  2.8624 & 3.6096 \\
\midrule
\textbf{ar} & 3.5546 & 3.7510 & 4.7967 & 3.7568 & 4.0791 & 3.2360 & 3.1133 & 2.7075 &2.7315 &3.0873 & 3.7821\\
\textbf{de} & 3.8861 & 3.5092 & 4.9626 & 3.9055 & 4.1539 & 3.3429 & 3.1189 & 2.8173 & 2.7535 & 3.0852 & 3.9186 \\
\textbf{en} & 3.8742 & 3.8270 & 4.6347 & 3.8585 & 4.2320 & 3.3177 & 3.1034  & 2.8129 & 2.7436 & 3.0899 & 3.9407 \\
\textbf{es} & 3.8339 & 3.7929  & 4.8842 & 3.6712 & 4.1942 & 3.2895 & 3.0974 & 2.7693 & 2.7569 & 3.1046 & 3.8816\\
\textbf{fa} & 3.7464 & 3.6334 & 4.7350 & 3.6938 & 3.8038 & 3.1910 & 3.0848 & 2.6704 & 2.7339 & 3.0595 & 3.7303 \\
\textbf{fr} & 3.8722 & 3.8528 & 4.9441 & 3.8526 & 4.1329 & 3.0936 & 3.1116 & 2.8150 & 2.7406 &3.1577 &3.9641 \\
\textbf{hi} & 3.8431 & 3.7554 & 4.8606 & 3.8120 & 4.2017 & 3.2725 & 2.8757 & 2.7432 & 2.7612 & 3.1281 & 3.8329\\
\textbf{ru} & 3.8820 & 3.8683 & 5.0007 & 3.9182 & 4.1466 & 3.3656 & 3.0847 & 2.5907 & 2.7566 & 3.1553 & 3.9728 \\
\textbf{sw} & 3.8650 & 3.7613 & 4.8704 & 3.8184 & 4.2288 & 3.2863 & 3.1022 & 2.7505  & 2.4657  & 3.0666 & 3.8442 \\
\textbf{ur} & 3.8644 & 3.7545 & 4.8701 & 3.8153 & 4.1892 & 3.2778 & 3.0937 & 2.7456 & 2.7575 & 2.8638 & 3.8410 \\
\textbf{zh} & 3.8852 & 3.8804 & 5.0004 & 3.9216 & 4.1565 & 3.3698 & 3.1025 & 2.8302 & 2.7675 & 3.1015 & 3.5754 \\






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  en  & 4.7140 & 4.7089 & 5.0786 & 5.0970 & 5.1289 &5.1441 & 5.0102\\
%  fr &  3.2118 & 3.4158 & 3.1967 & 3.4430 & 3.4788 & 3.4735 & 3.3792\\ 
%  de & 3.6441 & 3.9567 & 3.9784 & 3.6480 & 4.0204 & 4.0032 & 3.9113\\
%  zh & 3.7305 & 4.0634 & 4.0886  & 4.0907  & 3.7058 & 4.0951 & 3.9958\\ 
%  ru & 2.6697 & 2.8977 & 2.8997 & 2.8983 & 2.9165 & 2.6559 & 2.8509\\
%  es & 3.7425 & 3.9757 & 3.9623 & 4.0235 & 4.0533 & 4.0413 & 3.7301\\
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  en  & 68.14 & 68.10 & 66.93 & 66.87 & 66.76 & 66.74 & 67.15  \\
%  fr &  74.98 & 73.79 & 74.95 & 73.67 & 73.50 & 73.54 & 74.03 \\ 
%  de & 72.36 & 70.85 & 70.75  &  72.37 &  70.60 &  70.70 & 71.09 \\
%  zh & 71.59 & 70.01 & 69.10 & 69.91 & 71.60 & 69.88 & 70.29 \\ 
%  ru &  78.24 & 76.61 & 76.60  & 76.59 & 76.49 & 78.37 & 76.92 \\
%  es & 71.88  & 70.75  & 70.83  & 70.58  & 70.41  & 70.48  & 71.87 \\

\midrule
\end{tabular}
}
\caption{Performance~(perplexity) of winning tickets at $50\%$ sparsity for the MLM task.}
\label{table:mlm_result_all}
\end{table*}

==> LTH_Multilingual_LMs_EMNLP/tables/MLM_winning_tickets.tex <==
\begin{table}
\footnotesize
\centering
\begin{tabular}{ l| c |c | c }
\toprule
  & mBERT & Winning Ticket & Sparsity~(\%) \\
\midrule
 en & 68.14 & 68.10 & 50\\
 fr & 74.98 & 74.95 & 50\\ 
 de & 72.36  & 72.37 & 50\\
 zh & 71.59 & 71.60 & 50\\ 
 ru & 78.24 & 78.37 & 50\\
 es & 71.88 & 71.87 & 50\\
\midrule
\end{tabular}
\caption{Performance~(accuracy) of winning tickets on the MLM task at the highest sparsity for which iterative pruning finds them.}
\label{table:mlm_result}
\vspace{-3mm}
\end{table}

==> LTH_Multilingual_LMs_EMNLP/tables/NER_cross_lang.tex <==
\begin{table*}[t]
\footnotesize
\centering
\begin{tabular}{ l c c c c c c c c c }
\toprule
\textbf{Model /} & & \multicolumn{8}{c}{\textbf{Target Language}} \\
  \textbf{Sub-network} & \textbf{ar} & \textbf{de} & \textbf{en} & \textbf{es} & \textbf{fa} & \textbf{fr} & \textbf{ru} & \textbf{ur} & \textbf{zh}\\
\midrule
\textbf{mBERT} & 88.64 & 89.11 & 83.47 & 91.11 & 92.33 & 90.51 & 89.39 & 95.31 & 79.53\\
\midrule
\textbf{ar} & 88.50 & 87.59 & 82.92 & 90.39 & 91.73 & 89.84 & 88.34 & 94.67 & 76.97\\
\textbf{de} & 87.09 & 88.81 & 83.06 & 90.43 & 91.20 & 89.59 & 88.38 & 93.93 & 77.25\\
\textbf{en} & 87.21 & 87.53 & 83.60 & 90.44 & 91.23 & 89.67 & 88.47 & 93.93 & 76.92\\
\textbf{es} & 87.10 & 87.59 & 83.10 & 91.08 & 91.33 & 89.93 & 88.25 & 94.22 & 76.51\\
\textbf{fa} & 87.47 & 87.55 & 82.73 & 90.18 & 92.25 & 89.59 & 88.34 & 94.10 & 76.73\\
\textbf{fr} & 87.33 & 87.81 & 82.85 & 90.56 & 91.40 & 90.31 & 88.50 & 94.42 & 76.72\\
\textbf{ru} & 87.26 & 87.84 & 82.99 & 90.43 & 91.41 & 89.75 & 89.03 & 94.35 & 76.96\\
\textbf{ur} & 86.81 & 87.35 & 82.59 & 90.08 & 91.35 & 89.50 & 87.94 & 96.44 & 76.73\\
\textbf{zh} & 86.94 & 87.48 & 82.42 & 90.11 & 91.17 & 89.47 & 88.21 & 93.65 & 79.33\\




%  \textbf{en}  & 83.47 & 83.65 & 82.83 & 82.53 & 82.45 & 82.77 & 82.79 & 82.92\\ 
%  \textbf{fr} & 90.51 & 89.78 & 90.42 & 89.68 & 89.56 & 89.46 & 89.81 & 89.54\\ 
%  \textbf{fa} & 92.33 & 91.26 & 91.39 & 92.25 & 91.02 & 91.23 & 91.87 & 91.23\\ 
%  \textbf{zh} & 79.56 & 76.83 & 76.69 & 76.79 & 79.47 & 76.85 & 77.27 & 77.10\\ 
%  \textbf{ur} & 95.52 & 93.37 & 94.26 & 93.91 & 93.93 & 96.47 & 94.86 & 93.84\\ 
%  \textbf{ar} & 88.69 & 87.23 & 87.41 & 87.56 & 87.01 & 86.96 & 88.50 & 87.04\\
%  \textbf{de} & 89.08 & 87.52 & 87.83 & 87.57 & 87.67 & 87.28 & 87.65 & 89.01\\

\midrule
%   \hline
\end{tabular}
\caption{Performance~(F1-score) of winning tickets at $50\%$ sparsity for the NER task.}
\label{table:ner_result_all}
% \vspace{-8mm}
\end{table*}

==> LTH_Multilingual_LMs_EMNLP/tables/NER_winning_tickets.tex <==
\begin{table}
\footnotesize
\centering
\begin{tabular}{ l| c |c| c  }
\toprule
  & mBERT & Winning Ticket & Sparsity~(\%)\\
\midrule
 en & 82.1 & 83.5 & 60\\
 fr & 90.4 & 90.4 & 60\\ 
 fa & 92.5  & 92.6 & 60\\
 zh & 79.5 & 79.6 & 50\\ 
 ur & 95.3 & 96.2 & 60\\
 ar & 88.6 & 88.7 & 50\\
 de & 89.0 & 89.0 & 50\\
\midrule
\end{tabular}
\caption{Performance~(F1-score) of winning tickets on the NER task at the highest sparsity for which iterative pruning finds them.}
\label{table:ner_result}
\vspace{-4mm}
\end{table}

==> LTH_Multilingual_LMs_EMNLP/tables/XNLI_cross_lang.tex <==
\begin{table*}[t]
\footnotesize
\centering
\begin{tabular}{ l c c c c c c c c c c }
\toprule
\textbf{Model /} & \multicolumn{10}{c}{\textbf{Target Language}} \\
% \midrule
\textbf{Sub-network}  & \textbf{ar} & \textbf{de} & \textbf{en} & \textbf{es}  & \textbf{fr} & \textbf{hi} & \textbf{ru} & \textbf{sw} & \textbf{ur} & \textbf{zh} \\
\midrule
\textbf{mBERT}  & 70.26 & 77.33 & 82.16 & 78.80 & 78.00 & 68.48 & 72.98 & 66.28 & 63.06 & 76.60\\
\midrule
    \textbf{ar} & 70.29 & 76.72 & 82.00 & 79.07 & 77.06 & 67.58 & 72.96 & 67.48 & 64.68 & 76.88\\
    \textbf{de} & 70.22 & 77.10 & 82.44 & 79.09 & 77.73 & 68.11 & 73.35 & 65.40 & 64.03 & 76.50 \\
    \textbf{en} & 71.17 & 77.12 & 82.14 & 79.73 & 78.23 & 67.90 & 74.38 & 66.37 & 64.03 & 76.66\\
    \textbf{es} & 70.57 & 77.42 & 82.43 & 79.15 & 77.36 & 68.06 & 74.31 & 64.97 & 63.61 & 76.98 \\
    \textbf{fr} & 70.52 & 76.96 & 82.80 & 79.56 & 77.61 & 68.39 & 73.31 & 66.77 & 63.85 & 77.31 \\
    \textbf{hi} & 70.94 & 76.24 & 82.54 & 77.96 & 77.15 & 68.04 & 72.93 & 65.78 & 64.07 & 76.50\\
    \textbf{ru} & 70.33 & 76.05 & 82.69 & 79.49 & 77.54 & 68.55 & 73.31 & 65.62 & 63.37 & 76.52 \\
    \textbf{sw} & 69.76 & 76.42 & 81.50 & 77.45 & 76.75 & 67.84 & 72.36 & 66.14 & 63.39 & 76.18 \\
    \textbf{ur} & 69.11 & 75.17 & 80.81 & 77.65 & 75.71 & 66.98 & 72.20 & 65.33 & 62.14 & 75.82\\
    \textbf{zh} & 69.79 & 76.16 & 81.45 & 78.73 & 77.80 & 67.74 & 72.67 & 65.51 & 63.85 & 76.01\\
% \begin{tabular}{ l c c c c c c c c}
% \toprule
% \textbf{Model /} & & \multicolumn{6}{c}{\textbf{Target Language}} \\
% \textbf{Sub-network} & \textbf{en} & \textbf{fr} & \textbf{ar}  & \textbf{ur} & \textbf{zh} & \textbf{sw} & \textbf{hi}\\
% \midrule
% \textbf{mBERT} & 82.16 & 78 & 70.41 & 63.06 & 77.03 & 66.1 & 68.48 \\
% \midrule
% \textbf{en} & 82.14 & 78.31 & 71.48 & 63.53 & 76.95 & 66.62 & 68.57 \\
% \textbf{fr} & 83.33 & 77.96 & 70.80 & 63.65 & 77.30 & 66.90 & 68.55 \\
% \textbf{ar} & 82.53 & 77.38 & 70.74 & 64.65 & 77.18 & 67.51 & 68.03 \\
% \textbf{ur} & 81.40 & 76.38 & 69.63 & 62.42 & 76.22 & 66.00 & 67.06 \\
% \textbf{zh} & 81.88 & 78.19 & 71.08 & 63.23 & 76.80 & 66.34 & 68.07 \\
% \textbf{sw} & 81.28 & 77.38 & 70.10 & 63.49 & 76.10 & 66.20 & 68.23 \\
% \textbf{hi} & 83.09 & 77.87 & 71.12 & 63.61 & 76.62 & 66.18 & 68.27 \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%  en  & 82.16 & 82.14 & 83.33 & 82.53 & 81.40 & 81.88 & 81.28 & 83.09 \\ 
%  fr  & 78.00 & 78.31 & 77.96 & 77.38 & 76.38 & 78.19 & 77.38 & 77.87\\ 
%  ar  & 70.41 & 71.48 & 70.80 & 70.74 & 69.63 & 71.08 & 70.10 & 71.12\\ 
%  ur  & 63.06 & 63.53 & 63.65 & 64.65 & 62.42 & 63.23 & 63.49 & 63.61\\ 
%  zh  & 77.03 & 76.95 & 77.30 & 77.18 & 76.22 & 76.80 & 76.1 & 76.62\\ 
%  sw  & 66.10 & 66.62 & 66.90 & 67.51 & 66.00 & 66.34 & 66.20 & 66.18\\
%  hi  & 68.48 & 68.57 & 68.55 & 68.03 & 67.06 & 68.07 & 68.23 & 68.27\\
 
 

\midrule
%   \hline
\end{tabular}
\caption{Performance~(accuracy) of winning tickets at $50\%$ sparsity for the XNLI task.}
\label{table:xnli_result_all}
% \vspace{-8mm}
\end{table*}

==> LTH_Multilingual_LMs_EMNLP/tables/XNLI_winning_tickets.tex <==
\begin{table}
\footnotesize
\centering
\begin{tabular}{l|c|c|c}
\toprule
  & mBERT & Winning Ticket & Sparsity~(\%)\\
\midrule
 en & 82.4 & 82.3 & 50\\
 fr & 78.2 & 78.2 & 50\\ 
 ar & 70.7 & 70.8 & 50\\
 ur & 63.2 & 62.7 & 30\\
 zh & 76.7 & 76.8 & 50\\ 
 sw & 66.1 & 66.2 & 50\\
 hi & 68.5 & 68.6 & 50\\
\midrule
\end{tabular}
\caption{Performance~(accuracy) of winning tickets on the XNLI task at the highest sparsity for which iterative pruning finds them.}
\label{table:xnli_result}
\vspace{-4mm}
\end{table}

% \footnote{Based on the LTH definition, this is not a winning ticket as it doesn't reach the full model performance}

==> LTH_Multilingual_LMs_EMNLP/tables/all_tasks_winning_ticket.tex <==
\begin{table*}[t]
% \footnotesize
\begin{center}
% \begin{small}
% \def\arraystretch{1.2}

\resizebox{\textwidth}{!}{\begin{tabular}{l|rrrr rrrr rrrr}
\toprule
\multicolumn{1}{c}{} & \multicolumn{4}{c}{\textbf{MLM (Perplexity)}} & \multicolumn{4}{c}{\textbf{NER (F1)}} & \multicolumn{4}{c}{\textbf{XNLI (Accuracy)}}\\
\cmidrule(lr){2-5}                   \cmidrule(lr){6-9}     \cmidrule(lr){10-13}      
% \midrule
 \multicolumn{1}{c}{} & \textbf{mBERT} & $f^*$ & $s$~(\%) &  \multicolumn{1}{r}{\textbf{rand}} & \textbf{mBERT} & $f^*$ & $s$~(\%) & \multicolumn{1}{r}{\textbf{rand}} & \textbf{mBERT} & $f^*$ & $s$~(\%) & \textbf{rand}\\
\toprule

ar & 3.5247 & 3.5546 & 50 & 6.4001  & 88.64 & 88.50 & 50 & 72.43 & 70.26 & 70.29 & 50 & 61.48 \\
de & 3.5143 & 3.5092 & 50 & 9.6489  & 89.11 & 88.81 & 50 & 75.68 & 77.33 & 77.10 & 50 & 65.98 \\
en & 4.6523 & 4.6347 & 50 & 10.9182 & 83.47 & 83.60 & 50 & 68.05 & 82.16 & 82.14 & 50 & 74.49 \\
es & 3.6775 & 3.6712 & 50 & 8.3084  & 91.11 & 91.08 & 50 & 79.44 & 78.80 & 78.93 & 60 & 67.67  \\
fa & 3.8033 & 3.8038 & 50 & 7.3315  & 92.33 & 92.10 & 60 & 75.66 &    -  &   -   & -  &   -   \\
fr & 3.1151 & 3.0936 & 50 & 6.8504  & 90.51 & 90.31 & 50 & 77.61 & 78.00 & 77.61 & 50 & 69.11 \\
hi & 2.8728 & 2.8757 & 50 & 5.1345  &    -  &   -   & -  &    -  & 68.48 & 68.04 & 50 & 58.75 \\
ru & 2.5927 & 2.5907 & 50 & 6.1112  & 89.39 & 89.03 & 50 & 74.91 & 72.98 & 72.73 & 60 & 62.20  \\
sw & 2.5001 & 2.4657 & 50 & 4.292   &    -  &   -   & -  &    -  & 66.28 & 66.14 & 50 & 59.55 \\
ur & 2.8624 & 2.8638 & 50 & 5.0286  & 95.31 & 95.94 & 60 & 84.33 & 63.06 & 63.13 & 30 & 58.75 \\
zh & 3.6096 & 3.5754 & 50 & 8.4811  & 79.53 & 79.33 & 50 & 57.44 & 76.60 & 76.01 & 50 & 68.23 \\

 
\midrule
\end{tabular}
}
\caption{Performance of winning tickets~($f^*$) on the XNLI, NER, and MLM tasks at the highest sparsity~($s$) for which iterative pruning finds them.
We also report the performance of a random sub-network of mBERT (\textbf{rand}) at the same sparsity level as the winning ticket.}

\label{table:all_in_result}
\vspace{-4mm}
% \end{small}
\end{center}
\end{table*}


==> LTH_Multilingual_LMs_EMNLP/tables/combined_datasets.tex <==
\begin{table}
% \footnotesize
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{ l c c c c c}
\toprule
\textbf{Model /} & \multicolumn{5}{c}{\textbf{Target Language}} \\
% \midrule
\textbf{Sub-network}  & \textbf{ar} & \textbf{de} & \textbf{es} & \textbf{ru}  & \textbf{ur} \\
\midrule
\textbf{mBERT}  & 88.69 & 89.08 & 91.11 & 89.22 & 95.52\\
\midrule
\textbf{$f^*$ } & 88.5  & 89.01 & 91.08 & 89.03 & 96.44\\
\midrule
\textbf{en} & 87.23 & 87.52	& 90.44	& 88.47	& 93.93\\
\textbf{fa} & 87.56 & 87.57 & 90.18 & 88.34 & 94.10 \\
\textbf{fr} & 87.41	 & \textbf{87.83} & 90.56	 & \textbf{88.50}	 & 94.42\\
\textbf{zh} &  87.01 & 87.67 & 90.11 & 88.21 & 93.65\\
\textbf{en-fa-fr-zh} & \textbf{87.64} & 87.81 & \textbf{90.77} & 88.34 & \textbf{94.59} \\

\midrule
%   \hline
\end{tabular}
}
\caption{Performance (F1-score) of winning tickets at 50\% sparsity level for combining training datasets of en, fa, fr, and zh languages for the NER task.}
\vspace{-4mm}
\label{table:combined_datasets}
\end{table}

==> LTH_Multilingual_LMs_EMNLP/tables/cross_lang_transfer.tex <==
\begin{table*}[]
\footnotesize
  \centering
\begin{tabular}{ l| c |c c c c c c }
\toprule
  & mBERT & en & fr & de & zh & ru & es \\
\midrule
 en  & 68.14 & 68.10 & 66.93 & 66.87 & 66.76 & 66.74 & 67.15  \\
 fr &  74.98 & 73.79 & 74.95 & 73.67 & 73.50 & 73.54 & 74.03 \\ 
 de & 72.36 & 70.85 & 70.75  &  72.37 &  70.60 &  70.70 & 71.09 \\
 zh & 71.59 & 70.01 & 69.10 & 69.91 & 71.60 & 69.88 & 70.29 \\ 
 ru &  78.24 & 76.61 & 76.60  & 76.59 & 76.49 & 78.37 & 76.92 \\
 es & 71.88  & 70.75  & 70.83  & 70.58  & 70.41  & 70.48  & 71.87 \\

\midrule
\end{tabular}
\caption{Performance of winning tickets at $50\%$ sparsity level for MLM task. The last column indicates the average accuracy drop for each language.}
\label{table:mlm_result_all}
\end{table*}


\begin{table*}[]
\footnotesize
\centering
\begin{tabular}{ l| c |c c c c c c c}
\toprule
  & mBERT & en & fr & ar  & ur & zh & sw & hi\\
\midrule
 en & 82.4 & 82.3 & 83.0 & 82.5 & 81.4 & 82.1 & 82.0 & 83.0 \\ 
 fr  & 78.2 & 78.3 & 78.2 & 77.3 & 76.3 & 78.2 & 77.2 & 77.8 \\ 
 ar  & 70.8 & 71.5 & 70.8 & 70.9 & 69.6 & 71.0  & 70.1 & 71.1\\ 
 ur & 63.2 & 63.5 & 63.6 & 64.6 & 62.4 & 63.3 & 63.4 & 63.6 \\ 
 zh & 76.8 & 76.6 & 77.3 & 75.7 & 76.0 & 76.3 & 76.1 & 76.6\\ 
 sw & 66.1 & 66.6 & 66.9 & 67.5 & 66.0 & 66.3 & 66.2 & 66.1\\
 hi   & 68.7 & 68.2 & 68.6 & 68.0 & 67.0 & 68.0 & 68.2 & 68.1\\

\midrule
%   \hline
\end{tabular}
\caption{Performance of transferring winning tickets across languages at $50\%$ sparsity level for XNLI dataset.}
\label{table:xnli_result_all}
\end{table*}


\begin{table*}
\footnotesize
\centering
\begin{tabular}{ l| c |c c c c c c c c }
\toprule
  & mBERT & en & fr & fa & zh & ur & ar & de\\
\midrule
 en  & 0.821 & 0.835  & 0.828 & 0.825 & 0.824 & 0.827 & 0.829 & 0.829\\ 
 fr & 0.904 & 0.897 & 0.904 & 0.896 & 0.895 & 0.894 & 0.898 & 0.895\\ 
 fa & 0.925 & 0.912 & 0.913 & 0.926 & 0.910 & 0.912 & 0.918 & 0.912\\ 
 zh & 0.795 & 0.768 & 0.766 & 0.767 & 0.796 & 0.768 & 0.772 & 0.771\\ 
 ur & 0.953 & 0.933 & 0.942 & 0.943 & 0.937 & 0.962 & 0.948 & 0.938\\ 
 ar & 0.886 & 0.872 & 0.874 & 0.876 & 0.870 & 0.869 & 0.887 & 0.870\\
 zh & 0.890 & 0.880 & 0.878 & 0.875 & 0.876 & 0.872 & 0.876 & 0.890\\ 

\midrule
%   \hline
\end{tabular}
\caption{Performance of winning tickets at $50\%$ sparsity level for NER task.}
\label{table:ner_result_all}
\end{table*}

==> LTH_Multilingual_LMs_EMNLP/tables/experiment_setup.tex <==
\begin{table}[!ht]
\begin{center}
% \begin{small}
\def\arraystretch{1.2}

% \footnotesize

\resizebox{\columnwidth}{!}{
\begin{tabular}{ l | c c c}
\hline
 Dataset & MLM & NER & XNLI \\
 \hline
 \# Train Ex. & 1,600,000 & 20,000 & 392,702 \\ 
 \# Valid. Ex. & 30,000 & 10,000 & 2,490\\
 \# Epochs & 1 & 3  & 3\\
 \# Iters/Epoch & 100,000 & 625 & 12,270\\
  Batch Size & 16 & 32 & 32 \\
%   Learning Rate & $5 \times 10^{-5}$ &  $2 \times 10^{-5}$ & $5 \times 10^{-5}$\\ 
    Learning Rate & $5 \times 10^{-5}$ & $2 \times 10^{-5}$ & \begin{tabular}{@{}l@{}}
                   mbert: $5 \times 10^{-5}$\\
                   mt5:   $2 \times 10^{-4}$\\
                 \end{tabular} \\
  Eval. Metric & Perplexity & F1 & Accuracy \\
  Optimizer & \multicolumn{3}{ c }{Adam with $\epsilon = 1 \times 10^{-8}$}\\
  \hline
\end{tabular}
}

\caption{Details of pre-training and fine-tuning. Learning rate decays linearly from initial value to zero.}
\vspace{-5mm}
\label{table:train_details}
% \end{small}
\end{center}
\end{table}

==> LTH_Multilingual_LMs_EMNLP/tables/mlm_results.tex <==
\begin{table}[!htbp]
\centering
\begin{tabular}{ l| c |c  }
\toprule
  & mBERT & winning ticket   \\
\midrule
 en & 68.14 & 68.10 \\
 fr & 74.98 & 74.95\\ 
 de & 72.36  & 72.37 \\
 zh & 71.59 & 71.60\\ 
 ru & 78.24 & 78.37\\
 es & 71.88 & 71.87 \\
\midrule
\end{tabular}
\caption{Performance of winning tickets on MLM task at 50\% sparsity level that is the highest sparsity for which iterative pruning finds them.}
\label{table:mlm_result}
\end{table}

\begin{table*}[!htbp]
  \centering
\begin{tabular}{ l| c |c c c c c c }
\toprule
  & mBERT & en & fr & de & zh & ru & es \\
\midrule
 en  & 68.14 & 68.10 & 66.93 & 66.87 & 66.76 & 66.74 & 67.15  \\
 fr &  74.98 & 73.79 & 74.95 & 73.67 & 73.50 & 73.54 & 74.03 \\ 
 de & 72.36 & 70.85 & 70.75  &  72.37 &  70.60 &  70.70 & 71.09 \\
 zh & 71.59 & 70.01 & 69.10 & 69.91 & 71.60 & 69.88 & 70.29 \\ 
 ru &  78.24 & 76.61 & 76.60  & 76.59 & 76.49 & 78.37 & 76.92 \\
 es & 71.88  & 70.75  & 70.83  & 70.58  & 70.41  & 70.48  & 71.87 \\

\midrule
\end{tabular}
\caption{Performance of winning tickets at $50\%$ sparsity level for MLM task. The last column indicates the average accuracy drop for each language.}
\label{table:mlm_result_all}
\end{table*}




==> LTH_Multilingual_LMs_EMNLP/tables/mt5_XNLI_cross_lang.tex <==
\begin{table*}[!ht]
\footnotesize
\centering
\begin{tabular}{ l c c c c c c c c c c }
\toprule
\textbf{Model /} & \multicolumn{10}{c}{\textbf{Target Language}} \\
% \midrule
\textbf{Sub-network}  & \textbf{ar} & \textbf{de} & \textbf{en} & \textbf{es}  & \textbf{fr} & \textbf{hi} & \textbf{ru} & \textbf{sw} & \textbf{ur} & \textbf{zh} \\
\midrule
\textbf{mT5} & 74.17 & 78.52 & 83.13 & 79.64 & 80.14 & 69.98 & 75.56 & 70.00 & 63.25 & 75.10\\
\midrule
\textbf{ar} & 71.25 & 74.43 & 79.69 & 76.14 & 75.47 & 67.18 & 73.51 & 67.24 & 61.14 & 69.15\\
\textbf{de} & 69.94 & 75.71 & 80.31 & 76.94 & 76.60 & 66.93 & 74.57 & 67.00 & 60.70 & 70.09 \\
\textbf{en} & 69.97 & 76.02 & 80.64 & 77.41 & 76.36 & 67.58 & 75.12 & 67.38 & 61.62 & 68.76\\
\textbf{es} & 70.68 & 76.76 & 80.72 & 77.64 & 76.96 & 67.73 & 74.78 & 66.80 & 61.22 & 69.82 \\
\textbf{fr} & 70.49 & 75.76 & 79.66 & 76.67 & 76.59 & 66.93 & 74.66 & 69.43 & 60.21 & 69.00 \\
\textbf{hi} & 68.79 & 73.50 & 78.29 & 74.63 & 74.01 & 66.19 & 71.96 & 65.74 & 61.06 & 67.64\\
\textbf{ru} & 69.67 & 74.89 & 79.33 & 76.16 & 75.07 & 67.37 & 74.22 & 67.13 & 60.44 & 70.22 \\
\textbf{sw} & 69.96 & 74.60 & 79.53 & 75.65 & 74.93 & 66.32 & 73.31 & 67.22 & 60.41 & 67.45 \\
\textbf{ur} & 66.20 & 71.28 & 75.76 & 72.04 & 71.58 & 65.17 & 69.99 & 64.07 & 60.48 & 67.60\\
\textbf{zh} & 70.40 & 75.15 & 80.05 & 75.74 & 75.36 & 66.99 & 73.75 & 65.98 & 59.80 & 71.44\\
\textbf{rand} & 61.20 & 66.70 & 73.57 & 68.11 & 67.67 & 61.08 & 66.30 & 61.84 & 56.82 & 62.57\\

 

\midrule
%   \hline
\end{tabular}
\caption{Performance~(accuracy) of at $50\%$ sparsity for the XNLI task on the mT5 model.}
\label{table:mt5_xnli_result}
% \vspace{-8mm}
\end{table*}

==> LTH_Multilingual_LMs_EMNLP/tables/ner_results.tex <==

\begin{table}[!htbp]
\centering
\begin{tabular}{ l| c |c| c  }
\toprule
  & mBERT & winning ticket & Sparsity   \\
\midrule
 en & 0.821 & 0.823 & 60\% \\
 fr & 0.904 & 0.904 & 60\% \\ 
 fa & 0.925  & 0.926 & 60\%  \\
 zh & 0.795 & 0.796 & 50\%\\ 
 ur & 0.953 & 0.961 & 60\%\\
 ar & 0.886 & 0.887 & 50\%\\
 de & 0.890 & 0.890 & 50\%\\
\midrule
\end{tabular}
\caption{Performance of winning tickets on NER task at the highest sparsity for which iterative pruning finds them.}
\label{table:ner_result}
\end{table}

\begin{table*}[!htbp]
\centering
\begin{tabular}{ l| c |c c c c c c c c }
\toprule
  & mBERT & en & fr & fa & zh & ur & ar & de\\
\midrule
 en  & 0.821 & 0.835  & 0.828 & 0.825 & 0.824 & 0.827 & 0.829 & 0.829\\ 
 fr & 0.904 & 0.897 & 0.904 & 0.896 & 0.895 & 0.894 & 0.898 & 0.895\\ 
 fa & 0.925 & 0.912 & 0.913 & 0.926 & 0.910 & 0.912 & 0.918 & 0.912\\ 
 zh & 0.795 & 0.768 & 0.766 & 0.767 & 0.796 & 0.768 & 0.772 & 0.771\\ 
 ur & 0.953 & 0.933 & 0.942 & 0.943 & 0.937 & 0.962 & 0.948 & 0.938\\ 
 ar & 0.886 & 0.872 & 0.874 & 0.876 & 0.870 & 0.869 & 0.887 & 0.870\\
 zh & 0.890 & 0.880 & 0.878 & 0.875 & 0.876 & 0.872 & 0.876 & 0.890\\ 

\midrule
%   \hline
\end{tabular}
\caption{Performance of winning tickets at $50\%$ sparsity level for NER task.}
\label{table:ner_result_all}
\end{table*}



==> LTH_Multilingual_LMs_EMNLP/tables/xnli_results.tex <==
\begin{table}[!htbp]
\centering
\begin{tabular}{l|c|c}
\toprule
  & mBERT & winning ticket   \\
\midrule
 en & 82.4 & 82.3\\
 fr & 78.2 & 78.2\\ 
 ar & 70.8  & 70.9  \\
 ur & 63.2 & - \\
 zh & 76.8 & 76.3\\ 
 sw & 66.1 & 66.2\\
 hi & 68.7 & 68.1\\
\midrule
\end{tabular}
\caption{Performance of winning tickets on XNLI task at the highest sparsity for which iterative pruning finds them.}
\label{table:xnli_result}
\end{table}

\begin{table*}[!htbp]
\centering
\begin{tabular}{ l| c |c c c c c c c}
\toprule
  & mBERT & English & French & Arabic  & Urdu & Chinese & Swahili & Hindi\\
\midrule
 English & 82.4 & 82.3 & 83.0 & 82.5 & 81.4 & 82.1 & 82.0 & 83.0 \\ 
 French  & 78.2 & 78.3 & 78.2 & 77.3 & 76.3 & 78.2 & 77.2 & 77.8 \\ 
 Arabic  & 70.8 & 71.5 & 70.8 & 70.9 & 69.6 & 71.0  & 70.1 & 71.1\\ 
 Urdu & 63.2 & 63.5 & 63.6 & 64.6 & 62.4 & 63.3 & 63.4 & 63.6 \\ 
 Chinese & 76.8 & 76.6 & 77.3 & 75.7 & 76.0 & 76.3 & 76.1 & 76.6\\ 
 Swahili & 66.1 & 66.6 & 66.9 & 67.5 & 66.0 & 66.3 & 66.2 & 66.1\\
 Hindi   & 68.7 & 68.2 & 68.6 & 68.0 & 67.0 & 68.0 & 68.2 & 68.1\\

\midrule
%   \hline
\end{tabular}
\caption{Performance of transferring winning tickets across languages at $50\%$ sparsity level for XNLI dataset.}
\label{table:xnli_result_all}
\end{table*}



==> tables/MLM_winning_tickets.tex <==
\begin{table}
\footnotesize
\centering
\begin{tabular}{ l| c |c | c }
\toprule
  & mBERT & Winning Ticket & Sparsity~(\%) \\
\midrule
 en & 68.14 & 68.10 & 50\\
 fr & 74.98 & 74.95 & 50\\ 
 de & 72.36  & 72.37 & 50\\
 zh & 71.59 & 71.60 & 50\\ 
 ru & 78.24 & 78.37 & 50\\
 es & 71.88 & 71.87 & 50\\
\midrule
\end{tabular}
\caption{Performance~(accuracy) of winning tickets on the MLM task at the highest sparsity for which iterative pruning finds them.}
\label{table:mlm_result}
\vspace{-3mm}
\end{table}

==> tables/NER_winning_tickets.tex <==
\begin{table}
\footnotesize
\centering
\begin{tabular}{ l| c |c| c  }
\toprule
  & mBERT & Winning Ticket & Sparsity~(\%)\\
\midrule
 en & 82.1 & 83.5 & 60\\
 fr & 90.4 & 90.4 & 60\\ 
 fa & 92.5  & 92.6 & 60\\
 zh & 79.5 & 79.6 & 50\\ 
 ur & 95.3 & 96.2 & 60\\
 ar & 88.6 & 88.7 & 50\\
 de & 89.0 & 89.0 & 50\\
\midrule
\end{tabular}
\caption{Performance~(F1-score) of winning tickets on the NER task at the highest sparsity for which iterative pruning finds them.}
\label{table:ner_result}
\vspace{-4mm}
\end{table}

==> tables/XNLI_winning_tickets.tex <==
\begin{table}
\footnotesize
\centering
\begin{tabular}{l|c|c|c}
\toprule
  & mBERT & Winning Ticket & Sparsity~(\%)\\
\midrule
 en & 82.4 & 82.3 & 50\\
 fr & 78.2 & 78.2 & 50\\ 
 ar & 70.7 & 70.8 & 50\\
 ur & 63.2 & 62.7 & 30\\
 zh & 76.7 & 76.8 & 50\\ 
 sw & 66.1 & 66.2 & 50\\
 hi & 68.5 & 68.6 & 50\\
\midrule
\end{tabular}
\caption{Performance~(accuracy) of winning tickets on the XNLI task at the highest sparsity for which iterative pruning finds them.}
\label{table:xnli_result}
\vspace{-4mm}
\end{table}

% \footnote{Based on the LTH definition, this is not a winning ticket as it doesn't reach the full model performance}

==> tables/cross_lang_transfer.tex <==
\begin{table*}[]
\footnotesize
  \centering
\begin{tabular}{ l| c |c c c c c c }
\toprule
  & mBERT & en & fr & de & zh & ru & es \\
\midrule
 en  & 68.14 & 68.10 & 66.93 & 66.87 & 66.76 & 66.74 & 67.15  \\
 fr &  74.98 & 73.79 & 74.95 & 73.67 & 73.50 & 73.54 & 74.03 \\ 
 de & 72.36 & 70.85 & 70.75  &  72.37 &  70.60 &  70.70 & 71.09 \\
 zh & 71.59 & 70.01 & 69.10 & 69.91 & 71.60 & 69.88 & 70.29 \\ 
 ru &  78.24 & 76.61 & 76.60  & 76.59 & 76.49 & 78.37 & 76.92 \\
 es & 71.88  & 70.75  & 70.83  & 70.58  & 70.41  & 70.48  & 71.87 \\

\midrule
\end{tabular}
\caption{Performance of winning tickets at $50\%$ sparsity level for MLM task. The last column indicates the average accuracy drop for each language.}
\label{table:mlm_result_all}
\end{table*}


\begin{table*}[]
\footnotesize
\centering
\begin{tabular}{ l| c |c c c c c c c}
\toprule
  & mBERT & en & fr & ar  & ur & zh & sw & hi\\
\midrule
 en & 82.4 & 82.3 & 83.0 & 82.5 & 81.4 & 82.1 & 82.0 & 83.0 \\ 
 fr  & 78.2 & 78.3 & 78.2 & 77.3 & 76.3 & 78.2 & 77.2 & 77.8 \\ 
 ar  & 70.8 & 71.5 & 70.8 & 70.9 & 69.6 & 71.0  & 70.1 & 71.1\\ 
 ur & 63.2 & 63.5 & 63.6 & 64.6 & 62.4 & 63.3 & 63.4 & 63.6 \\ 
 zh & 76.8 & 76.6 & 77.3 & 75.7 & 76.0 & 76.3 & 76.1 & 76.6\\ 
 sw & 66.1 & 66.6 & 66.9 & 67.5 & 66.0 & 66.3 & 66.2 & 66.1\\
 hi   & 68.7 & 68.2 & 68.6 & 68.0 & 67.0 & 68.0 & 68.2 & 68.1\\

\midrule
%   \hline
\end{tabular}
\caption{Performance of transferring winning tickets across languages at $50\%$ sparsity level for XNLI dataset.}
\label{table:xnli_result_all}
\end{table*}


\begin{table*}
\footnotesize
\centering
\begin{tabular}{ l| c |c c c c c c c c }
\toprule
  & mBERT & en & fr & fa & zh & ur & ar & de\\
\midrule
 en  & 0.821 & 0.835  & 0.828 & 0.825 & 0.824 & 0.827 & 0.829 & 0.829\\ 
 fr & 0.904 & 0.897 & 0.904 & 0.896 & 0.895 & 0.894 & 0.898 & 0.895\\ 
 fa & 0.925 & 0.912 & 0.913 & 0.926 & 0.910 & 0.912 & 0.918 & 0.912\\ 
 zh & 0.795 & 0.768 & 0.766 & 0.767 & 0.796 & 0.768 & 0.772 & 0.771\\ 
 ur & 0.953 & 0.933 & 0.942 & 0.943 & 0.937 & 0.962 & 0.948 & 0.938\\ 
 ar & 0.886 & 0.872 & 0.874 & 0.876 & 0.870 & 0.869 & 0.887 & 0.870\\
 zh & 0.890 & 0.880 & 0.878 & 0.875 & 0.876 & 0.872 & 0.876 & 0.890\\ 

\midrule
%   \hline
\end{tabular}
\caption{Performance of winning tickets at $50\%$ sparsity level for NER task.}
\label{table:ner_result_all}
\end{table*}

==> tables/mlm_results.tex <==
\begin{table}[!htbp]
\centering
\begin{tabular}{ l| c |c  }
\toprule
  & mBERT & winning ticket   \\
\midrule
 en & 68.14 & 68.10 \\
 fr & 74.98 & 74.95\\ 
 de & 72.36  & 72.37 \\
 zh & 71.59 & 71.60\\ 
 ru & 78.24 & 78.37\\
 es & 71.88 & 71.87 \\
\midrule
\end{tabular}
\caption{Performance of winning tickets on MLM task at 50\% sparsity level that is the highest sparsity for which iterative pruning finds them.}
\label{table:mlm_result}
\end{table}

\begin{table*}[!htbp]
  \centering
\begin{tabular}{ l| c |c c c c c c }
\toprule
  & mBERT & en & fr & de & zh & ru & es \\
\midrule
 en  & 68.14 & 68.10 & 66.93 & 66.87 & 66.76 & 66.74 & 67.15  \\
 fr &  74.98 & 73.79 & 74.95 & 73.67 & 73.50 & 73.54 & 74.03 \\ 
 de & 72.36 & 70.85 & 70.75  &  72.37 &  70.60 &  70.70 & 71.09 \\
 zh & 71.59 & 70.01 & 69.10 & 69.91 & 71.60 & 69.88 & 70.29 \\ 
 ru &  78.24 & 76.61 & 76.60  & 76.59 & 76.49 & 78.37 & 76.92 \\
 es & 71.88  & 70.75  & 70.83  & 70.58  & 70.41  & 70.48  & 71.87 \\

\midrule
\end{tabular}
\caption{Performance of winning tickets at $50\%$ sparsity level for MLM task. The last column indicates the average accuracy drop for each language.}
\label{table:mlm_result_all}
\end{table*}




==> tables/ner_results.tex <==

\begin{table}[!htbp]
\centering
\begin{tabular}{ l| c |c| c  }
\toprule
  & mBERT & winning ticket & Sparsity   \\
\midrule
 en & 0.821 & 0.823 & 60\% \\
 fr & 0.904 & 0.904 & 60\% \\ 
 fa & 0.925  & 0.926 & 60\%  \\
 zh & 0.795 & 0.796 & 50\%\\ 
 ur & 0.953 & 0.961 & 60\%\\
 ar & 0.886 & 0.887 & 50\%\\
 de & 0.890 & 0.890 & 50\%\\
\midrule
\end{tabular}
\caption{Performance of winning tickets on NER task at the highest sparsity for which iterative pruning finds them.}
\label{table:ner_result}
\end{table}

\begin{table*}[!htbp]
\centering
\begin{tabular}{ l| c |c c c c c c c c }
\toprule
  & mBERT & en & fr & fa & zh & ur & ar & de\\
\midrule
 en  & 0.821 & 0.835  & 0.828 & 0.825 & 0.824 & 0.827 & 0.829 & 0.829\\ 
 fr & 0.904 & 0.897 & 0.904 & 0.896 & 0.895 & 0.894 & 0.898 & 0.895\\ 
 fa & 0.925 & 0.912 & 0.913 & 0.926 & 0.910 & 0.912 & 0.918 & 0.912\\ 
 zh & 0.795 & 0.768 & 0.766 & 0.767 & 0.796 & 0.768 & 0.772 & 0.771\\ 
 ur & 0.953 & 0.933 & 0.942 & 0.943 & 0.937 & 0.962 & 0.948 & 0.938\\ 
 ar & 0.886 & 0.872 & 0.874 & 0.876 & 0.870 & 0.869 & 0.887 & 0.870\\
 zh & 0.890 & 0.880 & 0.878 & 0.875 & 0.876 & 0.872 & 0.876 & 0.890\\ 

\midrule
%   \hline
\end{tabular}
\caption{Performance of winning tickets at $50\%$ sparsity level for NER task.}
\label{table:ner_result_all}
\end{table*}



==> tables/xnli_results.tex <==
\begin{table}[!htbp]
\centering
\begin{tabular}{l|c|c}
\toprule
  & mBERT & winning ticket   \\
\midrule
 en & 82.4 & 82.3\\
 fr & 78.2 & 78.2\\ 
 ar & 70.8  & 70.9  \\
 ur & 63.2 & - \\
 zh & 76.8 & 76.3\\ 
 sw & 66.1 & 66.2\\
 hi & 68.7 & 68.1\\
\midrule
\end{tabular}
\caption{Performance of winning tickets on XNLI task at the highest sparsity for which iterative pruning finds them.}
\label{table:xnli_result}
\end{table}

\begin{table*}[!htbp]
\centering
\begin{tabular}{ l| c |c c c c c c c}
\toprule
  & mBERT & English & French & Arabic  & Urdu & Chinese & Swahili & Hindi\\
\midrule
 English & 82.4 & 82.3 & 83.0 & 82.5 & 81.4 & 82.1 & 82.0 & 83.0 \\ 
 French  & 78.2 & 78.3 & 78.2 & 77.3 & 76.3 & 78.2 & 77.2 & 77.8 \\ 
 Arabic  & 70.8 & 71.5 & 70.8 & 70.9 & 69.6 & 71.0  & 70.1 & 71.1\\ 
 Urdu & 63.2 & 63.5 & 63.6 & 64.6 & 62.4 & 63.3 & 63.4 & 63.6 \\ 
 Chinese & 76.8 & 76.6 & 77.3 & 75.7 & 76.0 & 76.3 & 76.1 & 76.6\\ 
 Swahili & 66.1 & 66.6 & 66.9 & 67.5 & 66.0 & 66.3 & 66.2 & 66.1\\
 Hindi   & 68.7 & 68.2 & 68.6 & 68.0 & 67.0 & 68.0 & 68.2 & 68.1\\

\midrule
%   \hline
\end{tabular}
\caption{Performance of transferring winning tickets across languages at $50\%$ sparsity level for XNLI dataset.}
\label{table:xnli_result_all}
\end{table*}


